Estimating Buildings' Parameters over Time Including Prior Knowledge

Modeling buildings' heat dynamics is a complex process which depends on various factors including weather, building thermal capacity, insulation preservation, and residents' behavior. Gray-box models offer a causal inference of those dynamics expressed in few parameters specific to built environments. These parameters can provide compelling insights into the characteristics of building artifacts and have various applications such as forecasting HVAC usage, indoor temperature control monitoring of built environments, etc. In this paper, we present a systematic study of modeling buildings' thermal characteristics and thus derive the parameters of built conditions with a Bayesian approach. We build a Bayesian state-space model that can adapt and incorporate buildings' thermal equations and propose a generalized solution that can easily adapt prior knowledge regarding the parameters. We show that a faster approximate approach using variational inference for parameter estimation can provide similar parameters as that of a more time-consuming Markov Chain Monte Carlo (MCMC) approach. We perform extensive evaluations on two datasets to understand the generative process and show that the Bayesian approach is more interpretable. We further study the effects of prior selection for the model parameters and transfer learning, where we learn parameters from one season and use them to fit the model in the other. We perform extensive evaluations on controlled and real data traces to enumerate buildings' parameter within a 95% credible interval.

==> Background.tex <==
\section{Background}
\label{sec:Background}
   A grey-box modeling approach combines physical knowledge with statistical modeling. In this approach, we posit a probabilistic model, and perform statistical inference to learn the model's parameters from data.  In this section we explain statistical inference for probabilistic models, our intuition for choosing the Bayesian approach to inference, and we provide background on thermal building models.



%\subsection{Bayesian Statistics for Modeling}
\subsection{Statistical Inference}
   \label{subsec:Bayes}
     The two paradigms of statistical learning are the \textit{frequentist} and \textit{Bayesian} approaches. %, which are two different ways of solving a problem.
\emph{Maximum likelihood estimation} (MLE), a frequentist's choice for parameter estimation, does not incorporate any prior beliefs but rather infers parameters, e.g. building quality parameters, directly from the data.
%For a latent variable model, where the evidence is given by Y. %JF: sentence fragment, removed
Given the observed evidence $Y$, the MLE of the parameters $\theta$ is a \emph{point estimate} (i.e. a single value),
%   \begin{eqnarray}\label{eqn:MLE}
%     MLE = arg max_{\theta} P(X; \theta | Y)
%     \end{eqnarray}
%JF: The above equation is not correct. See below:

   \scriptsize
\begin{eqnarray}\label{eqn:MLE}
     \hat{\theta}_{MLE} = arg  \enspace  max_{\theta} P(Y; \theta) \mbox{ .}
\end{eqnarray}

   \normalsize
Here, $P(Y;\theta)$ is known as the \emph{likelihood}.  In practice, it is typically more convenient to equivalently maximize the \emph{log-likelihood}, $\log P(Y; \theta)$.
When the model posits additional latent variables $X$, $P(Y; \theta) = \int P(Y,X; \theta) dX$, and the optimization can be performed using the expectation maximization (EM) algorithm, which further outputs a distribution over the latent variables $P(X| Y;\theta)$. 
In frequentist statistics, probabilities are interpreted as the long-run frequencies of events when repeatedly performing an experiment under similar conditions.  Hence, under the frequentist approach the parameters $\theta$, and indeed the choice of the true model generating the data $M$, cannot be considered to be random variables, i.e. we cannot define a distribution $P(\theta)$ or $P(M)$. Instead, the model $M^*$ and its parameters $\theta^*$ are understood to be constant but unknown quantities.  As such, the performance of parameter estimation and model selection, which cannot take into account uncertainty over parameters, becomes heavily dependent on the sample size, due to vulnerability to overfitting.
%JF: I removed the comment about hypothesis tests, since there are other ways to do frequentist model selection, e.g. AIC.
The other drawback of the frequentist approach is that confidence intervals do not provide the probability that $\theta$ is in a given range (which a frequentist considers to be undefined), but rather the probability that the confidence interval procedure would capture the parameters, if repeated many times.  Hence, the most probable values for the parameters,  which are important for building parameter modeling, are not ascertained. 

Alternatively, Bayesian analysis is a statistical methodology that allows one to consider prior beliefs about a population parameter $\theta$ with evidence from a data sample to guide the statistical inference process. In Bayesian statistics, probabilities are defined to be \emph{degrees of belief} given available evidence.  Thus, unlike in frequentist statistics, parameters $\theta$, and even models $M$, may be random variables.  A prior probability distribution $P(\theta)$ for the parameters of interest $\theta$ is specified first. The evidence $Y$ is then obtained and combined through an application of Bayes' theorem to provide a posterior probability distribution for the parameters, $P(\theta|Y)$. The posterior distribution provides the basis for statistical inferences concerning the parameters. Bayesian parameter estimation can be performed using maximum a posteriori estimation (MAP), which obtains a point estimate at the mode of the posterior distribution.
%      \begin{eqnarray}\label{eqn:MAP}
%     MAP = arg max_{X;\theta} P(X; \theta | Y)P(X; \theta)
%     \end{eqnarray}
%JF: The above is slightly wrong, corrected below.

   \scriptsize
\begin{align}\label{eqn:MAP}
     \hat{\theta}_{MAP} = arg \enspace   max_{\theta} P( \theta | Y) &= arg \enspace  max_{\theta} \enspace   P(Y| \theta)  P(\theta)\\
     &= arg \enspace   max_{\theta} \enspace   \log P(Y| \theta)  + \log P(\theta) \nonumber
\end{align}
   \normalsize
   
The MAP is a point estimate of the parameters $\theta$ based on empirical data $Y$ and prior beliefs $P(\theta)$.  
It is similar to MLE but employs an augmented optimization objective which adds the log of the prior distribution, $\log P(\theta)$, to the quantity one otherwise wants to optimize, $\log P(Y;\theta)$.\footnote{The frequentist notation $P(Y;\theta)$ treats $\theta$ as a parameter, while the Bayesian notation $P(Y|\theta)$ treats $\theta$ as a random variable, but these are otherwise equivalent.} MAP estimation can therefore be seen as a regularization of ML estimation. MAP estimation is not fully Bayesian, as it provides a point estimate for the parameters rather than the full posterior distribution. Fully Bayesian inference aims to recover the posterior $P(\theta|Y)$ or $P(X,\theta|Y)$, thereby fully accounting for uncertainty.  %, generally comes with a heavy computational cost.
The posterior distribution is given by Bayes' rule.  
% \begin{equation} \label{eqn:posterior}
% P(X ; \theta| Y) = \frac{P( Y | X; \theta) P(X; \theta)}{\int_{X; \theta} P(Y,X; \theta)}
% \end{equation}
%JF: corrected the above.

   \scriptsize
\begin{equation} \label{eqn:posterior}
 P(X, \theta| Y) = \frac{P( Y | X, \theta) P(X, \theta)}{\int_{X, \theta} P(Y,X, \theta) dX d\theta} 
\end{equation}
   \normalsize
   
%JF: Don't put blank space between equations and surrounding text.  This adds unnecessary white space around the equations :)
The denominator of Equation~\ref{eqn:posterior} is $P(Y)$, the marginal probability of the data, which is found by marginalizing out the hidden variables and parameters from the joint distribution.
%An MLE or MAP approach is equivalent to approximating the posterior at a single snapshot of the model parameters.
This integral is often intractable, in which case exact inference is computationally infeasible, leading to the use of approximate inference techniques such as Markov chain Monte Carlo or variational inference~\cite{blei2017variational,jordan1999introduction}.
%Variational inference technique to approximate the posterior distribution and get a faster solution than MCMC approaches, which estimates the model over a range of parameters. %JF: removed this sentence, as it is stated elsewhere and not needed here.



\subsection{Thermal Dynamics for Buildings}
Grey-box modeling begins by designing a model.  
Previous works have described buildings' thermal dynamics with equivalent lumped electrical models. They were formulated by a set of first order stochastic differential equations which were solved with a Kalman Filter, to obtain the building parameters.
We take the example of the $T_iT_e$ model to illustrate grey-box modeling. The RC circuit equivalent of the $T_iT_e$ model is shown in Fig~\ref{fig:TiTe}, which describes the different parts of the building. The model has two states $T_i$ and $T_e$, where $T_i$ is the indoor temperature and $T_e$ is the building envelope temperature. We define \textbf{R}, \textbf{C}, and \textbf{A} to be the set of resistances, capacitances and solar infiltration for individual models. For example, in the $T_iT_e$ model \{\textbf{R}: $R_{ie},R_{ea}$\} are the set of all the resistance parameters. The stochastic differential equation is given by:
      
      \scriptsize
   \begin{flalign}
   dT_i &= \frac{1}{R_{ie}C_i} (T_e - T_i) dt + \frac{1}{C_i}\Phi_hdt + \frac{A_w }{C_i}\Phi_s dt +  \sigma_i d\omega_i \\
   dT_e &= \frac{1}{R_{ie}C_e} (T_i - T_e) dt +  \frac{1}{R_{Bea}C_e} (T_a - T_e) dt   +  \sigma_e  d\omega_e \\
   Y_k &= T_{i_k} + e_k
   \end{flalign}
      \normalsize
      
   where \textit{t} is the time, \textit{$R_{ie}$} is the thermal resistance between the interior and the building envelope, \textit{$R_{ea}$} is the thermal resistance between the building envelope and the ambient air, $C_i$ is the heat capacity of the interior, $C_e$ is the heat capacity of the building envelope, $\Phi_h$ is the energy flux from the heating system, $A_w$ is the effective window area, $\Phi_s$ is the energy flux from solar radiation, Ta is the ambient air temperature, $\{\omega_{i,t}\}$ and $\{\omega_{e,t}\}$ are standard Wiener processes with covariances $\Sigma_i$ and $\Sigma_e$  respectively, where t is the point in time t of a measurement, $Y_t$ is the measured interior temperature and $e_k$ is the measurement error, which is assumed to be a Gaussian white noise process.  A more general representation of the state space model can is given by 
   
      \scriptsize
   \begin{flalign}
     X_{n+1} &= A X_{n}    + B U_{n}   +  \sigma_w \label{eqn:state} \\
     Y_{n} &= C X_{n} + \sigma_v \label{eqn:estimation}
   \end{flalign}
      \normalsize
      
 where A is the state transition model, C is the observation model,  B is the control-input model which is applied to the control vector U, and Y is the observed values. Converting the differential equations (Eqns 1-3) as a difference equations we get the transition and emission matrix form as: 
 
    \scriptsize
  \begin{flalign}
   \begin{bmatrix} Ti(t+1) \\ Te(t+1)\end{bmatrix} &=
\begin{bmatrix}
    1 -  \frac{1}{R_{ie}C_i}    &  \frac{1}{R_{ie}C_i}   \\
   \frac{1}{R_{ie}C_e}     &    1 -  \frac{1}{R_{ie}C_e} -  \frac{1}{R_{ia}C_e}  
\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix}  \nonumber \\ 
&+ \begin{bmatrix}
    0   &  \frac{1}{C_i} &   \frac{A_{w}}{C_i} \\
   \frac{1}{R_{ia}C_e}     &    0 & 0
\end{bmatrix}\times \begin{bmatrix} Ta(t+1) \\ \Phi_h(t+1) \\ \Phi_s(t+1) \end{bmatrix}  + \begin{bmatrix}
   \sigma_{i}    &  0   \\
   0   &    \sigma_{e}  
\end{bmatrix} \label{eqn:trans}  \\
     Y(t)  &=  \begin{bmatrix} 1 & 0\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix} + \sigma \label{eqn:emis}
  \end{flalign}
    \normalsize
 
Eqn~\ref{eqn:state}. is the state transition of the dynamic system, i.e $P(x_{t+1} | x_t)$ $\sim$ $\mathcal{N}(AX + BU, \Sigma_w)$, and Eqn~\ref{eqn:estimation}. is the observation probability which is given by  $P(y_{t} | x_t)$ $\sim$ $\mathcal{N}(CX , \Sigma_v)$. Assuming the Markov properties of the model and the Gaussian nature of the noise and initial distributions, the maximum a posteriori estimation (MAP) for a sequence of states is obtained by optimizing the posterior probability density:
 
    \scriptsize
  \begin{flalign} 
 P(\theta| Y) &\propto \prod_{i=1}^N P(y_k | Y_{k-1};\theta)P(\theta) = P(\theta) P(y_0;\theta)\prod_{i=1}^N P(y_k | y_{k-1};\theta)
  \end{flalign}
    \normalsize
    
  Here the observed variables are $Y$, and we maximize the above function with respect to parameters $\theta$.
  %Solving the above problem, parameters can be estimated using maximum a posteriori estimation, where the prior distribution of the parameters were considered to be Gaussian.
  Without any prior information (uniform priors), the problem reduces to maximum likelihood estimation. The MAP approximation of the solution to the problem is achieved using the extended Kalman filter as shown in~\cite{MADSEN199567, KRISTENSEN2004225}.  Both of the problems were solved by manually initializing the parameters and setting a pre-defined bound on the parameters. This ensured that the parameters lie within a range but point estimates were obtained without any error bounds for parameter prediction. 

\indent In~\cite{bacher2011identifying} lumped building models were constructed in an increasing order of complexity. The more complex models had more model parameters and likelihood ratio tests were performed to find the simplest best explanation of the building thermal dynamics. The primary model parameters are approximations of the home's total heat capacity and the thermal resistance, which measure the heat storage capacity and the insulation of the house, respectively. 
The above methods used point estimation techniques to recover building parameters.  In this work, we instead develop a fully Bayesian approach, in order to take parameter uncertainty into account in the inference process.





 
 
 
%%\subsection{Standard Building   Parameters}

%% We list some of the standard building model parameters that building inspectors use for assessing the quality of a building. As per Energy Star Home sealing recommendations, buildings should meet certain standards for insulation, infiltration or exfiltration, and the quality for windows and doors. Insulation for walls, ceilings, and floors is dependent climatic zones in of the location and the type of heating sources~\cite{star1october}. This is typically measured by \textbf{R-value}, which is a measure for how well an object per unit of it's exposed area resists flow of heat. The heat flow is governed by the temperature differential between the indoor and outdoor temperature.  Infiltration or exfiltration is measured for the air-leakage in a house, which is obtained using blower door test~\cite{sherman1995use}. The test quantifies the amount of leakage in a house in terms of metrics like Air Changes per hour at 50 Pascal pressure ($\mathbf{ACH_{50}}$). However, the measurements don't say where exactly are leaks present in the house. Energy auditors first determine whether a house require further inspection using blower door test and then check for leakages manually using thermal cameras. Thermal mass' describes a material's capacity to absorb, store and release heat. A common analogy is thermal mass as a kind of thermal battery. When heat is applied (to a limit) by radiation or warmer adjoining air, the battery charges up until which time it becomes fully charged. It discharges when heat starts to flow out as the adjoining air space becomes relatively cooler. It is used in the calculation of the Thermal Mass Parameter (\textbf{TMP}) which is the ratio between the sum of area times the heat capacity of construction materials and the total floor area. In terms of building lumped models, the R-value is similar to the resistance between the interior and exterior, the infiltration rate through convection is given by the $\mathbf{ACH_{50}}$ which is an additional resistance parameter and the TMP is the capacitance of the wall unit. 

 

==> EEnergy Arxiv/Analysis.tex <==
    
\begin{table*}[t]
\centering
\caption{Results of Study I}
\label{Table:Study1}
\begin{tabular}{@{}p{0.6cm}p{0.8cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.6cm}p{0.8cm}p{0.7cm}p{2.5cm}@{}}
\hline
Model                   & Method & Total R     & Total C                                                   & Ria         & Rie                                                      & Rih                                                     & Rea                                                    & Ci                                                       & Ce                                                       & Ch                                                        & Aw                                                     & Ae                                                    & NRMSE (\%) & RMSE        & Convergence Time (Steps) \\ \hline
\multirow{3}{*}{Ti}     & EKF     & 5.29        & 24.797                                                      & 5.29        &                     -                                     &      -                                                   &                                  -                      & 2.06                                                     &                                 -                         &       -                                                    & 7.89                                                    & -                                                      & 0.4        & 0.06        & 2.68s ( Steps = 39)               \\
                        & MCMC   & 5.29, 0.06  & 24.96,  0.36   & 5.29, 0.06  &                -                                          &                                      -                   &     -                                                   & 24.96, 0.36                      -                        &      -                                                    &                                               -            & 7.95, 0.675                                            &                                          -             & 0.8     & 0.10   &   30 min (Chains = 4, Steps = 5000)      \\
                        & ADVI   & 5.29, 0.67  & 24.75, 0.40    & 5.29, 0.067 &      -                                                    &                              -                           &   -                                                     & 24.73, 0.43                                    &  -                                                        &                                       -                    & 7.87, 0.675                                            &                                  -                     & 0.4       & 0.05       & 2.26min (Steps = 180000)         \\ \hline
\multirow{3}{*}{TiTe}   & EKF     & 5.36       & 39.17                                                      &      -       & 5.17                                                   &                               -                          &  0.19                                                    & 19.99                                                     & 19.18                                                  &       -                                                    & 23.78                                                  &   -                                                    & 0.3        & 0.04        & 14.65s  (100)            \\
                        & MCMC   & 5.27, 0.17  & 89.95,  7.92   &        -     & 1.73, 0.056                                              &                          -                               & 3.54, 0.122                                            & 21.39, 0.30                                              & 68.56, 7.91                                              &                 -                                          & 10.75, 0.64                                            &            -                                           & 0.3      & 0.04      &  1.5 hrs (4,5000)      \\
                        & ADVI   & 5.29, 0.002 & 25.31, 0.86   &       -      & 1.98, 0.001                                              &                               -                          & 3.31, 0.002                                            & 24.49 , 0.502                                            & 0.82, 0.008                                              &                      -                                     & 7.90, 0.86                                             &                  -                                     & 0.3      & 0.04       & 2:38 min (Steps =  180000)         \\ \hline
\multirow{3}{*}{TiTeTh} & EKF     &        -  & -                                                     &           -  &                                          -            &                  -                               &                              -                      &                  -                                   &                                      -               &                       -                         &    -                                               &    -                                                &    -    &  -    & No Convergence              \\\\
                        & MCMC   &       -      &             -                                              &          -   & 159.13, 273.83 & 70.23, 159.81 & 23.08, 68.44 & 119.77, 206.30 &  121.85, 184.87  &  313.33,   342.47  &  15.52,  28.71  &  0.092,  0.60 &     -       &    -         & No Convergence           \\
                        & ADVI   & 2.8, 0.004  &  184.45,   13.58 &     -        & 2.176, 0.010                                             & 0.23, 0.003                                             & 0.63, 0.003                                            & 177.82, 83.22                                            & 2.05, 0.03                                               & 4.59, 0.097                                               & 52.76, 193.86                                          & 45.50, 181.90                                         &   -     &      -   & 4.23min  (Steps = 180000)        \\ \hline
\end{tabular}
\end{table*}
 
 
  \section{{Analysis}} 
  \label{sec:Analysis}
  In this section we provide two case studies. In the first test case we compare the results with small dataset to contrast and compare the gray-box models' solutions with the Kalman filter and Bayesian state space model. In the second case study, we present results and analyses on larger scale data from the Dataport Dataset~\cite{Pecan}.
  
  \subsection{{Case Study I: Exploratory Study on a Benchmark Dataset}}
    \label{subsec:Case}
   
\subsubsection{Dataset} We compare the results with the benchmark dataset provided   in~\cite{bacher2011identifying} and the circuit assumptions of the house mentioned in the paper. The data is from a Flexhouse in Ris{\o} DTU in Denmark, and  was collected during a series of experiments carried out in February to April 2009, where measurements consist of five minute values over a period of six days. The dataset consist of a single signal representing the indoor temperature ($y$ $^{\circ}$C).  Observed ambient air temperature at the climate station ($Ta$ $^{\circ}$C).  Total heat input from the electrical heaters in the building ($\Phi_h$ kW). The global irradiance was measured at the climate station ($\Phi_s$ kW/$m^2$).

 \subsubsection{Problem Formulation}
 \label{subsec:ProbForm}
 
 First we constructed all the models suggested in~\cite{bacher2011identifying}. The  CTSM~\cite{kristensen2003continuous}  package can be used to model Continuous Time Stochastic Processes   which is realized using an Extended Kalman Filter (EKF).   We define \textbf{R}, \textbf{C}, and \textbf{A} to be the set of resistances, capacitances and area of solar infiltration for individual models. The three models which we chose for inspection and their system dynamics as follows: 
 \begin{itemize}
     \item \textit{Ti Model:} Here the house as a whole is assumed to have one thermal resistance ($R_{ia}$) and capacitance ($C_i$).
 
 \begin{flalign}
 T_i(k+1)  &=  (1 - \frac{1}{R_{ia}C_i}) \times T_i(k)  + \frac{1}{R_{ia}C_i} \times T_e(k+1)  \nonumber    \\ &+ \frac{1}{C_i} \times \Phi_h(k+1) + \frac{A_w }{C_i}\Phi_s(k+1) +  \sigma_i  \\
 Y_k &= T_i(k)  + e_k 
 \end{flalign}
 
 \item \textit{TiTe Model:}    We provided a detailed description of formulation using the TiTe model in Section~\ref{subsec:Problem}. 
 
 \item \textit{ TiTeTh Model:} The three state model represents the interior subscripted by i, the exterior subscripted by e  and the heater subscripted by h. The formulation for the three states are as follows:  
     

  \begin{flalign}
   T_i(k+1)  &=  (1 - \frac{1}{R_{ie}C_i}) \times T_i(k)  + \frac{1}{R_{ie}C_i}\times  T_e(k+1) \nonumber   \\  &+\frac{A_w }{C_i} \times  \Phi_s(k+1) + \sigma_i    \\
   T_e(k+1) &= (1-\frac{1}{R_{ie}C_e}-\frac{1}{R_{ea}C_e}) \times  T_e(k)  +  \frac{1}{R_{ea}C_e} \times  T_a(k+1) \nonumber   \\ &+ \frac{1}{R_{ie}C_e} \times  T_i(k+1) +  \sigma_e    \\
     T_h(k+1)  &=  (1 - \frac{1}{R_{ih}C_h}) \times  T_h(k) + \frac{1}{R_{ih}C_h} \times  T_i(k+1) \nonumber   \\  &+ \frac{1}{C_h} \times  \Phi_h(k+1) + \sigma_h   \\
   Y_k &= T_i(k)  + e_k 
   \end{flalign} 
 
 \end{itemize}
 
 
 \subsubsection{{Results Discussion}} We show the results 
 of the first case study in Table~\ref{Table:Study1}. We provide the \textbf{mean} and \textbf{variances} ($\mu$, $\sigma$) of the estimated model parameters --  \textbf{R}, \textbf{C} and \textbf{Aw}, within a 95\% credible interval range as shown in Table~\ref{Table:Study1}. The total \textbf{R} and total \textbf{C} the composite thermal resistance and capacitance of the building. We compare the results of Bayesian Inference with the point estimates with an Extended Kalman Filter (EKF). The insights from the study are as follows: \\
\indent \textbf{{\emph{Estimated model parameters:}}} From the Table~\ref{Table:Study1} we found that the mean of the credible interval for the estimated parameters for the Bayesian approaches is similar to that of the EKF point estimate. The EKF assumes the parameters to have uniform priors and thus performs MLE for estimation. An approximate ADVI provides a similar parameter estimation as that of an equivalent run of MCMC inference. \\
\indent \textbf{{\emph{Comparison with the point estimates:}}} A direct comparison of the model's performances between the Bayesian methods and the EKF is difficult. We take the mean of the parameter estimated from Bayesian inference and then perform a one-step-ahead prediction and compare that with the EKF. The metrics used for comparison are the root mean squared (RMSE) and the normalized root mean squared errors (NRMSE) of the one-step-ahead prediction and we find that estimates from ADVI give us the best results (Table~\ref{Table:Study1}). \\
\indent \textbf{{\emph{Time of execution to reach convergence:}}} MLE estimates of the EKF is the fastest as it does not require computation of the full posterior distribution, however, it does not provide estimation error over model parameters.  The MCMC algorithm is the most time consuming one, where we increase the number of steps and check for convergence using Gelman-Rubin diagnostic. We selected 4 chains and an initial burn in 5000 steps which is intended to give the Markov Chain time to reach its equilibrium distribution when there is a random initial starting point.  Compared to MCMC, ADVI is much faster. For the $TiTeTh$ model, we obtain no convergence for the EKF or MCMC, i.e. the credible intervals are very wide. But ADVI provides reasonable intervals for some parameters. We listed the time of execution for the different approaches in Table~\ref{Table:Study1}.  

 \begin{figure}[t] 
\begin{subfigure}{.35\textwidth}
\includegraphics[width=\textwidth]{figs/RollingADVITi}
\label{fig:RollingADVITi}
\caption{Ti model}
\end{subfigure}
\hfill
\begin{subfigure}{.35\textwidth}
\includegraphics[width=\textwidth]{figs/RollingADVITiTe}
\label{fig:RollingADVITiTe}
\caption{TiTe model}
\end{subfigure}
\caption{Monte Carlo Simulation of Indoor Temperature}
\label{fig:Sim}
\end{figure}


 \indent\textbf{{\emph{Monte-Carlo simulation:}}} We perform a Monte-Carlo simulation to generate the possible indoor temperature scenarios when weather and HVAC usage is provided. In Figure~\ref{fig:Sim} we show the results of the simulated prediction for the Ti and TiTe models, drawing samples from the inferred parameter distributions. We considered the starting state to be drawn from a $\mathbb{N}$(70, 5) distribution, i.e. our guess for the indoor temperature will be within the range of 60 - 80$^{\circ}$F. The simulated prediction shows that the actual value of the indoor temperature is enclosed within the credible region. It, however, deviates in certain sections, which we hypothesize is because the thermal mass of a house can change with varying temperature. The RC constant~\cite{boylestad2002electronic}  of the data changes with time as the thermal mass \textbf{C} of a house can vary, due expansion (or contraction) of air. A more generalized formulation of thermal dynamics will require exploring longitudinal studies that to correlate between the parameter and temperature changes with the heater and cooler usage for long duration. 
  \begin{figure}[t] 
\begin{subfigure}{.45\textwidth}
\includegraphics[width=\textwidth]{figs/HiddenTiTe}
\caption{Hidden States of TiTe  model}
\label{fig:HiddenTiTe}
\end{subfigure}
\hfill 
\begin{subfigure}{.5\textwidth}
\includegraphics[width=\textwidth]{figs/HiddenTiTeTh}
\caption{Hidden States of TiTeTh model}
\label{fig:HiddenTiTeTh}
\end{subfigure}
\caption{Visualizing Hidden State Dynamics}
\label{fig:Qual}
\end{figure}


 \begin{figure*}[t]
\centering     
\begin{subfigure}{.38\textwidth}
\includegraphics[width=\textwidth]{figs/SARIMAX}
\caption{ARIMAX}
\label{fig:ARIMAX}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
\includegraphics[width=\textwidth]{figs/ForecastTi}
\caption{Ti Model}
\label{fig:TiForecast}
\end{subfigure}
\begin{subfigure}{.3\textwidth}
\includegraphics[width=\textwidth]{figs/ForecastTiTe}
\caption{TiTe Model}
\label{fig:TiTeForecast}
\end{subfigure} 
\caption{Comparison of Forecasting}
\end{figure*}

\indent  \textbf{{\emph{Qualitative assessment of the hidden states:} }}In Figure~\ref{fig:Qual}, we show the learned hidden states of the two-state $TiTe$ and three state $TiTeTh$ model. For the $TiTe$ model shown in Fig~\ref{fig:HiddenTiTe}, show that the estimated hidden state for the envelope is sandwiched between the indoor temperature and the outdoor temperature and is more correlated with the indoor temperature. Whereas in the $TiTeTh$  model (Fig~\ref{fig:HiddenTiTeTh}) the envelope state is more correlated with the outdoor temperature. However, the heater's temperature is the same as that of the indoor temperature, which implies it does not capture an independent factor of the  hidden state space. The plots in Fig~\ref{fig:Qual} show the error margin of the hidden states  obtained from the highest posterior distribution.







 

  
 \indent \textbf{{\emph{Forecasting:}}}   We compared the forecasting results of the BSSM with an auto-regressive integrated moving average with exogenous variables (ARIMAX). We used the first 5 days for training the BSSM and learn the building parameters. We then used the learned parameters to obtain a day ahead forecast within 95\% prediction interval, as presented in Algorithm~\ref{alg:Forecast}.  Our assumption is that the heater stays in the same state as the last known state and assumed that the solar radiation and temperature data are available.  In Figures~\ref{fig:ARIMAX} --~\ref{fig:TiTeForecast} we show the output of forecasting for the ARIMAX, $Ti$ and $TiTe$ models. For quantitative evaluation we chose the mean absolute percentage error (MAPE) to find the error in mean of the forecast and calculated the percent of data within 95\% forecast interval as shown in Table~\ref{table:Forecast}. The mean forecast error is lower in case of the BSSM models as they better learn the dynamics of the process. However, as the model parameters have a narrow credible interval, the actual data lies outside the forecast interval in  but provides a narrower band for which the actual value partially lies outside the credible interval. In contrast, the forecasting result of ARIMAX has less correlation, although the actual forecast is within the confidence interval. 
 
\begin{table}
\centering
\caption{Results of Forecasting}
\begin{tabular}{|l|l|l|}
\hline
Method &  MAPE  & \% of data within 95\%\\ &&forecast interval \\ \hline
ARIMAX & 0.19 & 100\%\\ \hline
Ti Model & 0.05 & 78\% \\ \hline
TiTe Model & 0.04 & 79\%\\ \hline 
\end{tabular}
\label{table:Forecast}
\end{table} 
 


\input{CaseStudy3}






==> EEnergy Arxiv/Background.tex <==
\section{Background}
\label{sec:Background}
   A grey-box modeling approach combines physical knowledge with statistical modeling. In this approach, we posit a probabilistic model, and perform statistical inference to learn the model's parameters from data.  In this section we explain statistical inference for probabilistic models, our intuition for choosing the Bayesian approach to inference, and we provide background on thermal building models.



%\subsection{Bayesian Statistics for Modeling}
\subsection{Statistical Inference}
   \label{subsec:Bayes}
     The two paradigms of statistical learning are the \textit{frequentist} and \textit{Bayesian} approaches. %, which are two different ways of solving a problem.
\emph{Maximum likelihood estimation} (MLE), a frequentist's choice for parameter estimation, does not incorporate any prior beliefs but rather infers parameters, e.g. building quality parameters, directly from the data.
%For a latent variable model, where the evidence is given by Y. %JF: sentence fragment, removed
Given the observed evidence $Y$, the MLE of the parameters $\theta$ is a \emph{point estimate} (i.e. a single value),
%   \begin{eqnarray}\label{eqn:MLE}
%     MLE = arg max_{\theta} P(X; \theta | Y)
%     \end{eqnarray}
%JF: The above equation is not correct. See below:

   \scriptsize
\begin{eqnarray}\label{eqn:MLE}
     \hat{\theta}_{MLE} = arg  \enspace  max_{\theta} P(Y; \theta) \mbox{ .}
\end{eqnarray}

   \normalsize
Here, $P(Y;\theta)$ is known as the \emph{likelihood}.  In practice, it is typically more convenient to equivalently maximize the \emph{log-likelihood}, $\log P(Y; \theta)$.
When the model posits additional latent variables $X$, $P(Y; \theta) = \int P(Y,X; \theta) dX$, and the optimization can be performed using the expectation maximization (EM) algorithm, which further outputs a distribution over the latent variables $P(X| Y;\theta)$. 
In frequentist statistics, probabilities are interpreted as the long-run frequencies of events when repeatedly performing an experiment under similar conditions.  Hence, under the frequentist approach the parameters $\theta$, and indeed the choice of the true model generating the data $M$, cannot be considered to be random variables, i.e. we cannot define a distribution $P(\theta)$ or $P(M)$. Instead, the model $M^*$ and its parameters $\theta^*$ are understood to be constant but unknown quantities.  As such, the performance of parameter estimation and model selection, which cannot take into account uncertainty over parameters, becomes heavily dependent on the sample size, due to vulnerability to overfitting.
%JF: I removed the comment about hypothesis tests, since there are other ways to do frequentist model selection, e.g. AIC.
The other drawback of the frequentist approach is that confidence intervals do not provide the probability that $\theta$ is in a given range (which a frequentist considers to be undefined), but rather the probability that the confidence interval procedure would capture the parameters, if repeated many times.  Hence, the most probable values for the parameters,  which are important for building parameter modeling, are not ascertained. 

Alternatively, Bayesian analysis is a statistical methodology that allows one to consider prior beliefs about a population parameter $\theta$ with evidence from a data sample to guide the statistical inference process. In Bayesian statistics, probabilities are defined to be \emph{degrees of belief} given available evidence.  Thus, unlike in frequentist statistics, parameters $\theta$, and even models $M$, may be random variables.  A prior probability distribution $P(\theta)$ for the parameters of interest $\theta$ is specified first. The evidence $Y$ is then obtained and combined through an application of Bayes' theorem to provide a posterior probability distribution for the parameters, $P(\theta|Y)$. The posterior distribution provides the basis for statistical inferences concerning the parameters. Bayesian parameter estimation can be performed using maximum a posteriori estimation (MAP), which obtains a point estimate at the mode of the posterior distribution.
%      \begin{eqnarray}\label{eqn:MAP}
%     MAP = arg max_{X;\theta} P(X; \theta | Y)P(X; \theta)
%     \end{eqnarray}
%JF: The above is slightly wrong, corrected below.

   \scriptsize
\begin{align}\label{eqn:MAP}
     \hat{\theta}_{MAP} = arg \enspace   max_{\theta} P( \theta | Y) &= arg \enspace  max_{\theta} \enspace   P(Y| \theta)  P(\theta)\\
     &= arg \enspace   max_{\theta} \enspace   \log P(Y| \theta)  + \log P(\theta) \nonumber
\end{align}
   \normalsize
   
The MAP is a point estimate of the parameters $\theta$ based on empirical data $Y$ and prior beliefs $P(\theta)$.  
It is similar to MLE but employs an augmented optimization objective which adds the log of the prior distribution, $\log P(\theta)$, to the quantity one otherwise wants to optimize, $\log P(Y;\theta)$.\footnote{The frequentist notation $P(Y;\theta)$ treats $\theta$ as a parameter, while the Bayesian notation $P(Y|\theta)$ treats $\theta$ as a random variable, but these are otherwise equivalent.} MAP estimation can therefore be seen as a regularization of ML estimation. MAP estimation is not fully Bayesian, as it provides a point estimate for the parameters rather than the full posterior distribution. Fully Bayesian inference aims to recover the posterior $P(\theta|Y)$ or $P(X,\theta|Y)$, thereby fully accounting for uncertainty.  %, generally comes with a heavy computational cost.
The posterior distribution is given by Bayes' rule.  
% \begin{equation} \label{eqn:posterior}
% P(X ; \theta| Y) = \frac{P( Y | X; \theta) P(X; \theta)}{\int_{X; \theta} P(Y,X; \theta)}
% \end{equation}
%JF: corrected the above.

   \scriptsize
\begin{equation} \label{eqn:posterior}
 P(X, \theta| Y) = \frac{P( Y | X, \theta) P(X, \theta)}{\int_{X, \theta} P(Y,X, \theta) dX d\theta} 
\end{equation}
   \normalsize
   
%JF: Don't put blank space between equations and surrounding text.  This adds unnecessary white space around the equations :)
The denominator of Equation~\ref{eqn:posterior} is $P(Y)$, the marginal probability of the data, which is found by marginalizing out the hidden variables and parameters from the joint distribution.
%An MLE or MAP approach is equivalent to approximating the posterior at a single snapshot of the model parameters.
This integral is often intractable, in which case exact inference is computationally infeasible, leading to the use of approximate inference techniques such as Markov chain Monte Carlo or variational inference~\cite{blei2017variational,jordan1999introduction}.
%Variational inference technique to approximate the posterior distribution and get a faster solution than MCMC approaches, which estimates the model over a range of parameters. %JF: removed this sentence, as it is stated elsewhere and not needed here.



\subsection{Thermal Dynamics for Buildings}
Grey-box modeling begins by designing a model.  
Previous works have described buildings' thermal dynamics with equivalent lumped electrical models. They were formulated by a set of first order stochastic differential equations which were solved with a Kalman Filter, to obtain the building parameters.
We take the example of the $T_iT_e$ model to illustrate grey-box modeling. The RC circuit equivalent of the $T_iT_e$ model is shown in Fig~\ref{fig:TiTe}, which describes the different parts of the building. The model has two states $T_i$ and $T_e$, where $T_i$ is the indoor temperature and $T_e$ is the building envelope temperature. We define \textbf{R}, \textbf{C}, and \textbf{A} to be the set of resistances, capacitances and solar infiltration for individual models. For example, in the $T_iT_e$ model \{\textbf{R}: $R_{ie},R_{ea}$\} are the set of all the resistance parameters. The stochastic differential equation is given by:
      
      \scriptsize
   \begin{flalign}
   dT_i &= \frac{1}{R_{ie}C_i} (T_e - T_i) dt + \frac{1}{C_i}\Phi_hdt + \frac{A_w }{C_i}\Phi_s dt +  \sigma_i d\omega_i \\
   dT_e &= \frac{1}{R_{ie}C_e} (T_i - T_e) dt +  \frac{1}{R_{Bea}C_e} (T_a - T_e) dt   +  \sigma_e  d\omega_e \\
   Y_k &= T_{i_k} + e_k
   \end{flalign}
      \normalsize
      
   where \textit{t} is the time, \textit{$R_{ie}$} is the thermal resistance between the interior and the building envelope, \textit{$R_{ea}$} is the thermal resistance between the building envelope and the ambient air, $C_i$ is the heat capacity of the interior, $C_e$ is the heat capacity of the building envelope, $\Phi_h$ is the energy flux from the heating system, $A_w$ is the effective window area, $\Phi_s$ is the energy flux from solar radiation, Ta is the ambient air temperature, $\{\omega_{i,t}\}$ and $\{\omega_{e,t}\}$ are standard Wiener processes with covariances $\Sigma_i$ and $\Sigma_e$  respectively, where t is the point in time t of a measurement, $Y_t$ is the measured interior temperature and $e_k$ is the measurement error, which is assumed to be a Gaussian white noise process.  A more general representation of the state space model can is given by 
   
      \scriptsize
   \begin{flalign}
     X_{n+1} &= A X_{n}    + B U_{n}   +  \sigma_w \label{eqn:state} \\
     Y_{n} &= C X_{n} + \sigma_v \label{eqn:estimation}
   \end{flalign}
      \normalsize
      
 where A is the state transition model, C is the observation model,  B is the control-input model which is applied to the control vector U, and Y is the observed values. Converting the differential equations (Eqns 1-3) as a difference equations we get the transition and emission matrix form as: 
 
    \scriptsize
  \begin{flalign}
   \begin{bmatrix} Ti(t+1) \\ Te(t+1)\end{bmatrix} &=
\begin{bmatrix}
    1 -  \frac{1}{R_{ie}C_i}    &  \frac{1}{R_{ie}C_i}   \\
   \frac{1}{R_{ie}C_e}     &    1 -  \frac{1}{R_{ie}C_e} -  \frac{1}{R_{ia}C_e}  
\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix}  \nonumber \\ 
&+ \begin{bmatrix}
    0   &  \frac{1}{C_i} &   \frac{A_{w}}{C_i} \\
   \frac{1}{R_{ia}C_e}     &    0 & 0
\end{bmatrix}\times \begin{bmatrix} Ta(t+1) \\ \Phi_h(t+1) \\ \Phi_s(t+1) \end{bmatrix}  + \begin{bmatrix}
   \sigma_{i}    &  0   \\
   0   &    \sigma_{e}  
\end{bmatrix} \label{eqn:trans}  \\
     Y(t)  &=  \begin{bmatrix} 1 & 0\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix} + \sigma \label{eqn:emis}
  \end{flalign}
    \normalsize
 
Eqn~\ref{eqn:state}. is the state transition of the dynamic system, i.e $P(x_{t+1} | x_t)$ $\sim$ $\mathcal{N}(AX + BU, \Sigma_w)$, and Eqn~\ref{eqn:estimation}. is the observation probability which is given by  $P(y_{t} | x_t)$ $\sim$ $\mathcal{N}(CX , \Sigma_v)$. Assuming the Markov properties of the model and the Gaussian nature of the noise and initial distributions, the maximum a posteriori estimation (MAP) for a sequence of states is obtained by optimizing the posterior probability density:
 
    \scriptsize
  \begin{flalign} 
 P(\theta| Y) &\propto \prod_{i=1}^N P(y_k | Y_{k-1};\theta)P(\theta) = P(\theta) P(y_0;\theta)\prod_{i=1}^N P(y_k | y_{k-1};\theta)
  \end{flalign}
    \normalsize
    
  Here the observed variables are $Y$, and we maximize the above function with respect to parameters $\theta$.
  %Solving the above problem, parameters can be estimated using maximum a posteriori estimation, where the prior distribution of the parameters were considered to be Gaussian.
  Without any prior information (uniform priors), the problem reduces to maximum likelihood estimation. The MAP approximation of the solution to the problem is achieved using the extended Kalman filter as shown in~\cite{MADSEN199567, KRISTENSEN2004225}.  Both of the problems were solved by manually initializing the parameters and setting a pre-defined bound on the parameters. This ensured that the parameters lie within a range but point estimates were obtained without any error bounds for parameter prediction. 

\indent In~\cite{bacher2011identifying} lumped building models were constructed in an increasing order of complexity. The more complex models had more model parameters and likelihood ratio tests were performed to find the simplest best explanation of the building thermal dynamics. The primary model parameters are approximations of the home's total heat capacity and the thermal resistance, which measure the heat storage capacity and the insulation of the house, respectively. 
The above methods used point estimation techniques to recover building parameters.  In this work, we instead develop a fully Bayesian approach, in order to take parameter uncertainty into account in the inference process.





 
 
 
%%\subsection{Standard Building   Parameters}

%% We list some of the standard building model parameters that building inspectors use for assessing the quality of a building. As per Energy Star Home sealing recommendations, buildings should meet certain standards for insulation, infiltration or exfiltration, and the quality for windows and doors. Insulation for walls, ceilings, and floors is dependent climatic zones in of the location and the type of heating sources~\cite{star1october}. This is typically measured by \textbf{R-value}, which is a measure for how well an object per unit of it's exposed area resists flow of heat. The heat flow is governed by the temperature differential between the indoor and outdoor temperature.  Infiltration or exfiltration is measured for the air-leakage in a house, which is obtained using blower door test~\cite{sherman1995use}. The test quantifies the amount of leakage in a house in terms of metrics like Air Changes per hour at 50 Pascal pressure ($\mathbf{ACH_{50}}$). However, the measurements don't say where exactly are leaks present in the house. Energy auditors first determine whether a house require further inspection using blower door test and then check for leakages manually using thermal cameras. Thermal mass' describes a material's capacity to absorb, store and release heat. A common analogy is thermal mass as a kind of thermal battery. When heat is applied (to a limit) by radiation or warmer adjoining air, the battery charges up until which time it becomes fully charged. It discharges when heat starts to flow out as the adjoining air space becomes relatively cooler. It is used in the calculation of the Thermal Mass Parameter (\textbf{TMP}) which is the ratio between the sum of area times the heat capacity of construction materials and the total floor area. In terms of building lumped models, the R-value is similar to the resistance between the interior and exterior, the infiltration rate through convection is given by the $\mathbf{ACH_{50}}$ which is an additional resistance parameter and the TMP is the capacitance of the wall unit. 

 

==> EEnergy Arxiv/CaseStudy3.tex <==
 
\subsection{{Case Study II: Prior Selection \& Transfer Learning}} 

\label{subsec:Case2}

\subsubsection{{Dataset}} The Dataport dataset is a publicly available dataset, created by Pecan Street Inc, which contains building-level electricity data from 1000+ households. We performed our experiments on three single-family homes from Texas (\emph{dataid} = 484, 739, 1507) based on metadata availability and proper registration of indoor temperature and HVAC usage data. The metadata, which has information about 52 homes, provides a general understanding about the buildings and helps us create prior distributions over the R-values.  Here, House 739 does not have heating data available and the metadata does not include a measure for House 1507's R-value.  
\subsubsection{{Experimental setup}} In this case study we explore the effects of prior selection and transfer learning. The two processes are inherently tied together, since in the Bayesian approach, ``today's posterior becomes tomorrow's prior.'' Our approach here is to learn the parameters from the AC usage season, where data is more consistent, and transfer the learned parameters as priors to seasons when HVAC has typically no usage and/or operates in heating mode. We investigate the effect of three sets of priors:

\begin{itemize}
\item \textit{Informed Priors (Set 1):} We selected informed gamma priors. This is useful when we have some notion about the parameters' values such as an initial audit to estimate the R-value of a building. We select a strong prior on the R-value where the mean of the R-value is same as that of the estimate and the standard deviation is 1.  

\item \textit{Hyper Priors (Set 2):} In this set, we don't have a direct estimation regarding the buildings' parameters but have a vague understanding about the expected value from the metadata. We encode such beliefs by setting  a hyper-prior for the mean, that is sampled selected from a mixture of lognormal distributions. We empirically found that R-values are a mixture of lognormal distributions, conditioned on the year built and conditioned square foot, by performing a maximum likelihood estimate. The estimated parameters of the two lognormal distributions as shown in Fig~\ref{fig:hist}, are ($\mu_0$, $\sigma_0$) = (3.02, 0.59) and ($\mu_1$, $\sigma_1$) = (3.43, 0.50),  respectively. 

\item \textit{Uninformed Priors (Set 3):} Finally, in \textit{Set 3}, we chose \textit{uninformed} flat gamma priors for the R-values, where, we have no knowledge of the buildings' parameters.  In all three cases we set a flat gamma prior on the C-values.
\end{itemize} 
  
  


 
 
 \begin{table*}[h]
\centering
\caption{Results of Case Study II}
\begin{tabular}{@{}lllllllll@{}}
\toprule
Homes & HVAC Mode & R-Value & \multicolumn{2}{l}{Informed Priors} & \multicolumn{2}{l}{Hyper Priors} & \multicolumn{2}{l}{Uninformed Priors} \\ \midrule
 &  &  & R & C & R & C & R & C \\ \cmidrule(l){4-9} 
 & No Usage &  & 26, 0.02 & 85.92, 12 & 53.24, 14.99 & 81.6, 10.86 & 449.04, 431.90 & 80.82 , 10.71 \\
484 & AC & 26 & 26, 0.02 & 85.03 , 12.5 & 52.12, 15.33 & 80.81, 11.08 & 453.73, 428.96 & 80.25, 10.99 \\
 & Heater &  & 26, 0.02 & 132.44 , 12.79 & 75.87, 15.9 & 89.35, 11.7 & 343.63 , 276.16 & 81.48 , 11.73 \\
 & No Usage &  & 6.1, 0.23 & 73.15, 18.84 & 61.82, 14.46 & 15.43, 1.945 & 62.1 , 14.33 & 15.33, 2.005 \\
739 & AC & 6 & 6.1, 0.23 & 64.09, 20.7 & 58.88, 10.87 & 15.55, 1.79 & 59.47, 10.43 & 15.65, 1.84 \\
 & Heater &  & - & - & - & - & - & - \\
 & No Usage &  & - & - & 24.52, 0.215 & 103.4, 7.34 & 48.66, 20.91 & 107.42, 7.56 \\
1507 & AC & NA & - & - & 23.58, 0.215 & 103.52, 7.89 & 47.65, 21.95 & 107.88, 7.55 \\
 & Heater &  & - & - & 23.58, 0.23 & 104.65, 8.79 & 52.22, 26.62 & 108.84, 8.38 \\ \bottomrule
\end{tabular}
\label{table:BestParam}
\end{table*}



\indent For all three cases, we set an upper bound on the R-values to be 70, which we found from the metadata. We assign an uninformed gamma prior on the C values. For all cases, we initially estimate for the AC usage scenario and use the mean and variance of the estimated parameters to set the prior for the other seasons.  The sign of the heat flux, as provided in Eqn~\ref{eqn:trans}, is negative when AC is used and the HVAC is in cooling mode. We do not have an exact value for heater's flux but we use the furnace which provides the binary ``ON-OFF'' signal of the heater and multiply an extra unknown parameter $\Phi_h$ to estimate the heat flux. Similarly to the previous section, we estimate all parameters within a 95\% credible interval. We also varied the size of the dataset of sizes [200, 500, 1000, 2000, 5000].
\subsubsection{Results}    The prior selection directly influences the value of the parameters, parameter transfer and depends on the size of the dataset. A summary of the results is presented in Table~\ref{table:BestParam} for 2000 data points, which provides us the most likely parameter estimates. We present the result in the form of mean and the error margins i.e. ($\mu$, $\pm \epsilon$). We find that the Informed Priors provide us with the most consistent estimates both across size of the datasets and when we perform transfer learning. As shown in Fig~\ref{fig:ErrIn}, the informed parameters remain consistent with the change in the size of the dataset with very little margin of error ($\pm$ 1). Parameter transfer also works best when informed priors are applied (Fig~\ref{fig:ErrIn}), but can provide us different estimates when being transferred from AC usage to Heater usage seasons.  The hyper-priors reduce the margin of error when applied for smaller datasets. For example, in Fig~\ref{fig:ErrUn}, the R-values have large error margins when uninformed priors are chosen, which is significantly reduced when hyperpriors were used Fig~\ref{fig:ErrHp}.  

\subsubsection{Discussion} 


Information in the data overwhelms prior information not only when the size of the dataset is large, but also when the prior encodes relatively small information. For example in House 739 (Table~\ref{table:BestParam}), an approach using uninformed priors will try to get the best estimate that fits the data, but the parameters may not be accurate. For this case, a sharp prior centered around an initial estimate gives the best result. Uninformative priors are easily persuaded by data, while strongly informative ones may be more resistant. When the size of the dataset is small, hyperpriors effectively reduce the margin of error in parameter estimation Fig.~\ref{fig:ErrHp}.
 
% \jf{Convergence time in MCMC iterations, or in size of the dataset?  I don't think we have results showing the former, and it wouldn't match my intuition.  Assuming you mean the latter, can put a supporting reference to Figure 8 here.}
 
\subsection{General Recommendations}%Takeaways from the Studies} % \jf{From both studies, plural, right?} 

     Based on our studies, we recommend constructing a Bayesian state space model customized for the problem at hand, carefully selecting the system dynamics and  priors. We suggest using ADVI for parameter estimation as it provides similar estimates but is faster than MCMC. In realistic settings, it is better to perform an initial audit to determine the home's insulation parameters and fix an informed prior on the parameter set. We suggest to use informative priors, if enough metadata is available to set them reliably. However, if the objective is to monitor a large set of homes, we recommend setting a hyper prior based on the beliefs from a sample of the dataset. If the heat flux is known from the HVAC, learning from one season and applying it to another can improve estimation. %safely\jf{too strong a word?} learn from one season and apply it on another. 

 
 

==> EEnergy Arxiv/Conclusion.tex <==
 
\begin{figure*}[!htp] 
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Informed484R}
\caption{}
\end{subfigure}
\hfill 
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Informed484C}
\caption{}
\end{subfigure}
\caption{Informed Prior set on R-values}
\label{fig:ErrIn}
\end{figure*}

\begin{figure*}[!htp]
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Hyper484R}
\caption{}
\end{subfigure}
\hfill 
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Hyper484C}
\caption{}
\end{subfigure}
\caption{Hyper Prior set on R-values}
\label{fig:ErrHp}
\end{figure*}

\begin{figure*}[!htp]
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Uninformed484R}
\caption{}
\end{subfigure}
\hfill 
\begin{subfigure}{.48\textwidth}
\includegraphics[width=\textwidth]{figs/Uninformed484C}
\caption{}
\end{subfigure}
\caption{Uninformed set on R-values}
\label{fig:ErrUn}
\caption*{ \textmd{{These figures show the results of parameter estimation of R and C values for House 484 with varying data sizes and different prior selection.}}}
\end{figure*}
 
 
 
\section{Conclusion \& Future Work}
\label{sec:Conclusion}
 
 In this paper, we proposed and  systematically studied Bayesian statistical approaches to buildings' thermal parameter estimation. We developed a generalized state-space modeling framework that integrates building physics equations with a statistical model. The model estimates buildings' structural parameters which influence the indoor temperature conditioned on HVAC usage and weather factors. We contrast model learning using MCMC and ADVI algorithms and show that Variational Inference is faster and provides a similar estimation to MCMC. A visual inspection of the hidden states was employed to assess the model dynamics, and we found that merely increasing model complexity does not capture any significant factors of the thermal characteristics. We further showed the model's applications, such as simulating probable outcomes and forecasting the future. The effects of prior selection on the parameter estimation were studied in detail. We found that informed priors provide the best estimates, but when such information is not present prior beliefs can help to better learn the models. Also, we found that priors are key to transfer learning, and model parameters learned from one season can be used to model thermal dynamics under the condition that %exogenous data is available and are properly scaled
 properly scaled exogenous data is available. \\ 
   \indent The focus of our future research is in two directions.  We are presently instrumenting several homes with smart thermostats and temperature sensors. This study serves as a guide to large-scale analysis as we attempt to further incorporate air leakages and construct room level thermal behavior analysis. We plan to learn from the data that is being collected longitudinally and incorporate the learned models in NEST thermostats to monitor homes' condition continuously. Secondly,  we will focus on incorporating air-leakage into the framework and  correlating with standardized metrics such as $ACH_{50}$. Common air-infiltration models (e.g. LBL model~\cite{sherman1992superposition}), have complex non-linear characteristics for which we will explore non-linear state space models. 
   
% \indent We presented a proof of concept for a thermal imaging system in our prior work~\cite{lachut2017longitudinal}, which can longitudinally collect data. Due to battery constraints and privacy issues, we choose to monitor a home's condition longitudinally with our proposed approach and deploy sensors to test for leakage if we detect anomaly in the estimation.  The Bayesian approach leaves room for inclusion of more information which is not necessarily part of thermal equations but coming from other data, such as human activity, quality of walls, windows and doors, whether windows and doors are unconsciously left open, usage of  appliances, etc, which will be useful for continuous modeling. 
 % Prior works~\cite{iyengar2018watthome} have focused on city-scale identification of homes that flags homes with anomalous usage and inundates the probable reasons for estimated energy loss.  
 
 %We presented a proof of concept for a thermal imaging system in our prior work~\cite{lachut2017longitudinal}, which can longitudinally collect data. Due to battery constraints and privacy issues, we choose to monitor a home's condition longitudinally with our proposed approach and deploy sensors to test for leakage if we detect anomaly in the estimation.  The Bayesian approach leaves room for inclusion of more information which is not necessarily part of thermal equations but coming from other data, such as human activity, quality of walls, windows and doors, whether windows and doors are unconsciously left open, usage of  appliances, etc, which will be useful for continuous modeling.  
%\jf{Breaks double blind!  Hide this reference for the submission?!?}
 

==> EEnergy Arxiv/Data.tex <==
\begin{comment}
\section{Data Set Description}
\label{data}

\subsection{Pecan Street}
\label{data:pecan}

\subsection{Data Cleaning}
\label{data:clean}

\subsection{Imaging System}
\label{data:cam}

The imaging system, shown in Figure~\ref{data:cam:fig}, extends the work-in-progress system first described in \cite{lachut_longitudinal_2017} with important improvements. The imaging system consists of an in-home hardware unit for data collection and back-end server software for data processing and analysis. The camera unit periodically pans $360\degree$ taking simultaneous IR and RGB images at regular intervals through the scan then uploading those images. The server processes the images and analyzes them to detect energy wastage or leakage.

\begin{figure}
\begin{subfigure}[b]{0.28\textwidth}
\includegraphics[height=0.25\textheight,width=\textwidth,keepaspectratio]{figs/CameraSystemBlock.jpg}
\caption{}
\label{data:cam:fig:blk}
\end{subfigure}~\begin{subfigure}[b]{0.2\textwidth}
%\includegraphics[height=0.3\textheight,width=0.1\textwidth ]{figs/CameraUnit.jpg}
\includegraphics[height=0.25\textheight,width=\textwidth,keepaspectratio]{figs/placeholder.png}
\caption{}
\label{data:cam:fig:pic}
\end{subfigure}
\caption{(a) Block diagram of the IR Camera system. (b) A prototype camera unit.}
\label{data:cam:fig}
\end{figure}

The improvements to the camera unit, pictured in Figure improved the system's reliability over previous iterations. The unit still uses the MLX90621---a low-power, low-resolution, and relatively low-cost IR camera \cite{MLX}---the Raspberry Pi camera module \cite{pi_camera}, and a $5V$ stepper motor. The Raspberry Pi Zero of previous versions has been replaced with a Zero W, reducing complexity by bringing the Wi-Fi radio on board the single-board computer that controls the rotation and data collection of the camera unit.

The 3D printed housing of the camera unit has been redesigned as well. While it still holds the two cameras in a fixed positional relation to each other, the housing now incorporates a small IR emitter in the base and an IR detector in the rotating portion. This emitter-detector pair creates a fixed point of reference between the rotating and stable parts of the camera unit. After each $360\degree$ scan, the camera rotates in reverse to this fixed point. The two advantages of this are: (1) a consistent correlation between pixel location and physical location in a longitudinal series of scans and (2) the power connection from the base of the unit is unwound after every scan. The first helps in data analysis. The second allows continuous power delivery for longitudinal operation.

After each scan, the collected images are uploaded to our back-end server for processing. The images are uploaded with {\tt rsync} and privacy of the data in transit is assured by {\tt ssh}. (In future work, we would like to ensure data privacy during analysis as well as transmission. However, the market success of the Nest Dropcam, Amazon Cloud Cam, Google Clips, and other products suggest that privacy need not be an overriding concern.) Each scan collects 64 RGB images and 64 IR images, each RGB+IR pair separated from the next by a $5.625\degree$ angle. To complete the scan, return the camera to zero position, and upload the collected images takes up to 15 minutes. Therefore, we have set the camera unit to scan at a regular interval, four times per hour.

\begin{figure}
\includegraphics[width=0.48\textwidth,height=0.25\textheight,keepaspectratio]{figs/homograph.png}
\caption{An illustration of projecting the thermal image into the space of the visual image.}
\label{data:cam:hom}
\end{figure}

On the server, the pre-analysis image processing proceeds through several steps for each batch of 64 images from a scan. First, the raw values from the IR camera are processed into temperature readings. The temperatures for all 64 images are then normalized to the range $[0,255]$ where $0$ is the minimum temperature measured across the batch and $255$ is the maximum. These initial IR images are $4\times16$ pixels and must be mapped to physical space. This mapping process is enabled by the fixed spatial relation between the IR and RGB cameras. We measured the relative fields of view to determine a homography, which we use to project the infrared information into the space of the corresponding visual image. This projection is illustrated in Figure~\ref{data:cam:hom}.

Next, the RGB and IR images are prepared to be stitched into panoramas. This is a rotational panorama through a single plane, so each image must be cylindrically warped as described in \cite{shum1997panoramic}. Figure~\ref{data:cam:hom} illustrates that the fields of view of the IR and RGB cameras on the camera unit do not perfectly overlap. Therefore, we crop the images down to only the shared field of view. Because of the number of images we take, such cropping represents a trivial loss of information, if any. The crop is done after the cylindrical warp, because the warping is done relative to the center of the image, a value the changes in the cropping.

The construction of the IR panorama and of the RGB panorama is done using pyramid blending, based on the technique in \cite{opencv_pyr}, but generalized to an arbitrary number of images as long as the number of images and the relation between the images is known. This method of constructing a panorama is necessary to prevent sharp edges between stitched photographs from tricking image segmentation or object detection algorithms.

Since we know the angle of rotation between images, $5.625\degree$, the focal length of the RGB camera, and the resolution of the RGB camera, we can calculate the horizontal movement distance of the camera unit between sequential images of a scan as a number of pixels. This length is $\Delta_{px}$. The final output panorama will be as many pixels tall as our cropped input images and as many pixels wide as the width of an input image plus $63\Delta_{px}$ The first step in pyramid blending is to create a zeroed-out placeholder image of these dimensions for each of our input images. Each input image is then copied into its place in its placeholder---the first image of a scan into the leftmost area of its placeholder, the second into its place shifted to the right by $\Delta_{px}$, the third shifted by $2\Delta_{px}$, and so on.

Then, from each placeholder, we create a Gaussian and a Laplacian pyramid. A Gaussian pyramid is a series of images wherein an original image is reduced in size several times. When these images are re-expanded they are blurred relative to the image, having lost information in the size reduction. The Laplacian pyramid is constructed by re-expanding each smaller image to its previous size and subtracting it from the one-step-larger image from which the smaller image was made. The result of this subtraction is to highlight the edges in the image one step higher in the pyramid. The Laplacian pyramid is always one level shallower than the Gaussian pyramid from which it was made.

\begin{figure}
\includegraphics[width=0.5\textwidth,height=0.25\textheight]{figs/placeholder.png}
\caption{Samples of the RGB and IR panoramas created with the pyramid blending method.}
\label{data:cam:pan}
\end{figure}

At each level of the Laplacian pyramid, we then assemble all 64 images of that level. Using the NumPy {\tt hstack} function, each of the 64 images at each level gets its corresponding $1/64$ of the assembled image. The pyramid is then recombined from the bottom up. The smallest image in the Laplacian pyramid is expanded to the size of the next larger image. The two images are summed. This sum image is again expanded and summed with the next larger image. The process repeats until the final output size image is reached. This final output image, because of this combination blurring and sharpening procedure, is smooth without being blurry or losing its true colors. See Figure~\ref{data:cam:pan} for an example of this result.

%% Object detection?

%% Image segmentation?

%% Longitudinal analysis?



\end{comment} 

==> EEnergy Arxiv/Introduction.tex <==
\section{{Introduction}}
 Retrofitting an existing building often reduces its energy consumption and particularly the heating and cooling costs. To assess the effectiveness of the retrofit, auditors perform on-site tests to gauge the insulation and infiltration quality of a house. However, such tests are expensive and intrusive, and thus cannot be carried out continuously. The proliferation of smart thermostats %\jf{These are already here, right? I'd delete ``on the horizon''} 
 such as   NEST and Ecobee~\cite{KLEIMINGER2014493}, and their acceptance and deployment in home environments are opening up new research avenues. In the near term, we envision a self-adaptive and programmable thermostat, that can seamlessly receive environmental data from the indoor and outdoors, and residents' activities, to model the inherent thermal characteristics of the building. Such a dynamic and adaptive smart thermostat will provide an early assessment of the insulation and leakage, and thus help promote energy sensitive actions and maintain comfort levels. 
  
 \indent Physicists have studied methods for modeling buildings' thermal conditions by way of several measurable parameters~\cite{tarantola2005inverse,fabrizio2015methodologies}.  In these models, the  thermal dynamics of a building are represented by an RC-circuit, due to system equivalence,  which allows us to  derive a set of stochastic differential equations that describe the thermal patterns. The composite parameters \emph{resistance} (\textbf{R}) and \emph{capacitance} (\textbf{C}) of the circuit are analogous to the buildings' insulation (and to some extent the infiltration), and the thermal mass,  respectively. Building quality measurement uses standardized metrics such as R-value (or U-value) to measure insulation and $ACH_{50}$ to measure infiltration. The thermal mass of a house is the ability of a material to absorb and store heat energy. Optimization based techniques~\cite{Optimization,gouda2002building} are popularly used to estimate the parameters, where the objective is to reduce the error between observed and predicted values. However, most approaches do not simultaneously consider two key factors that are common in the real world:
    \begin{itemize}
   \item \textit{Stochasticity of the building parameters:} The optimization-based methods are effective for fitting a model to data, but cannot provide a margin of error on the estimation. This is important as stochasticity arises due to several unaccounted factors, including human activity and home appliance   usage, which cannot be directly quantified. 
\item \textit{Presence of prior knowledge:} It is common knowledge that older buildings have poor insulation. Studies~\cite{EIA} show that the  average  house size has increased with time, and that larger homes typically have better insulation quality. By incorporation of prior knowledge such as \textit{``How old is a building?''} or \textit{``How much square footage does it have?''}, these intuitions about a building's condition can potentially increase the accuracy of the estimated parameters.
\end{itemize}

  \indent  To address these concerns, the Bayesian approach is a natural and simple way to incorporate prior knowledge in the building thermal modeling framework which also approximates the factors influencing the model dynamics. It allows for comparisons among multiple candidate models instead of performing binary hypothesis tests on a single model. The Bayesian posterior distribution plays the role of Occam's razor, effectively penalizing an increase in model complexity, such as adding variables, while rewarding improvements in fit. However, the existing Bayesian approaches have a few notable limitations: \emph{(i)} Bayesian inference of the parameters is primarily performed with Markov Chain Monte Carlo (MCMC) algorithms~\cite{gordon1993novel, geweke2001bayesian} which take a long time to converge, and thus are not well suited for the case where model complexity and/or data size increase. \emph{(ii)} A majority of previous works applied uninformed normal priors and do not evaluate the effect of prior selection on model performance. As such the full benefit of a Bayesian statistical approach is not utilized. \emph{(iii)} Finally, most studies limit their scope to a single seasonal period, particularly in the winter when residents use the HVAC in heating mode, and do not study how the model parameters estimated in one season can be used to monitor the house longitudinally.
  \begin{figure}[h]
    \begin{subfigure}{.23\textwidth} \includegraphics[height=3.5cm,width=1\textwidth]{figs/HistogramHigh}
    \end{subfigure}
    \begin{subfigure}{.23\textwidth}  \includegraphics[height=3.5cm,width=1\textwidth]{figs/HistogramLow}
    \end{subfigure}     
    \caption{Distribution of R-values of houses}
    \label{fig:hist}
    \end{figure}  
    
 \indent  To investigate these shortcomings and their resolution, in this paper we present a systematic study of Bayesian approaches to the modeling of buildings' thermal dynamics. We propose a generalized Bayesian State Space Model (BSSM) that can combine physics-based thermal models into a probabilistic framework. We further embed prior intuition and knowledge regarding buildings into the model based on subjective beliefs. For example, in Figure~\ref{fig:hist}, the probability densities of the R-values of homes built before the year 2000 differ depending on their size, in this case whether their area is less than 2000 square feet. We show how to incorporate such knowledge by effective prior selection. However, such priors are not conjugate to the likelihood and solutions cannot be computed analytically. We thus perform inference based on algorithms that do not depend on conjugacy, such as Automatic Differentiation Variational Inference, and show that the buildings' parameters can be estimated effectively with such an approximate approach. We analyze the effect of learning parameters from one season and use transfer learning to estimate the thermal dynamics in a different season when the HVAC is used in a different mode. We present two case studies on real data traces to show the effectiveness of the Bayesian approach, and the effects of prior selection and transfer learning across seasons.\\
\indent \textbf{Key Contributions:} Our innovations and results provide evidence that the Bayesian approach to modeling a building's thermal characteristics is valuable. The primary contributions of our work are as follows.  
\begin{itemize}
  \item \textit{Bayesian State Space Model:}  We propose a  Bayesian state-space model for estimating buildings' thermal parameters.  Unlike previous methods~\cite{bacher2011identifying,juhl2017grey, EstimationBuildsys,  KRISTENSEN2004225}  which use point estimates, our Bayesian model is capable of incorporating beliefs using non-conjugate priors, and managing uncertainty in the parameters.  We inferred the model parameters within a 95\% credible interval with a Mean Field Variational Approximation, and show that the estimates are as accurate as that of a more time-consuming MCMC approach. 
 %  \item \textit{Fast Bayesian inference using Variational Inference algorithms:} %\jf{I normally wouldn't capitalize Variational Inference, as it's not a proper noun, but I did so here as it's capitalized elsewhere.  The most important thing is to be consistent across the whole paper.}
%
  \item \textit{Interpretable assessment of the generative model:}  We explored the generative characteristics of the model by Monte-Carlo simulation and forecasting, which helps understand the causal physical process that describes the thermal behavior of a house. We also tested the quality of the models by forecasting indoor temperature with the learned building parameters. 
 % \item \textit{Effect of prior selection:} We studied their behavior with rigorous experiments beliefs about a building's condition in the form of prior selection to further enrich the model. 
  \item \textit{Effects of transfer learning \& prior selection:} 
 We proposed a transfer learning based approach by learning buildings' parameters in summer, when HVAC is typically operational in cooling mode, and used it to aid fitting the data in seasons when HVAC is not used or operates in heating mode. We propose a systematic approach to prior selection to incorporate beliefs about the buildings' characteristics in the model and conducted rigorous experiments to study their behavior. 
    \end{itemize}
The rest of the paper is structured as follows. In Section~\ref{sec:Related} we discuss related work on building parameter identification and Bayesian estimation. In Section~\ref{sec:Model} we propose the Bayesian State Space model for building parameter identification. In Section~\ref{sec:Analysis} we present two case studies and provide analysis of the model and finally conclude in Section~\ref{sec:Conclusion}. 
 


==> EEnergy Arxiv/Model.tex <==


\section{{Proposed Approach}}\label{sec:Model}  We follow the iterative modeling approach known as \emph{Box's loop}~\cite{blei2014build}, shown in Fig.~\ref{fig:Box}, for estimating buildings' thermal parameters. The process starts with a collected and pre-processed dataset.  We propose a Bayesian state space model to frame the problem and estimate parameters using MCMC and Variational Inference. Finally, we test for model convergence and measure the goodness of fit.
  
\begin{figure}[h]
\includegraphics[scale=.20, width=.45\textwidth]{figs/overall}
\caption{Box's Loop}
\label{fig:Box}
\end{figure}
  

 
\subsection{{ Bayesian Linear State Space Model} } 

  The generalized linear state space models consist of a sequence of $M$-dimensional observations ($y_1$, $y_2$, ... $y_N$), assumed to be generated from latent $D$-dimensional states $X$ = ($x_1$, $x_2$, ... $x_N$) and control variables $U$ =  ($u_1$, $u_2$, ... $u_N$). The data $Y$ is generated by the following state space equations:
 
   \begin{eqnarray}
   x_n = A x_{n-1} + B u_{n-1} + \mathcal{N}(0,Q) \label{eqn:stateEvolution} \\
   y_n = C x_n +  \mathcal{N}(0,R) \mbox{ ,} \label{eqn:obs}
    \end{eqnarray}
    
where Eqn.~\ref{eqn:stateEvolution} is the state evolution equation (analogous to HMM state transition) and Eqn.~\ref{eqn:obs} is the observation or measurement equation (emission probability). The overall state transition probability is given as 



 \begin{eqnarray}
  P(X | A, B) = \mathcal{N}(x_0 | m_0, \Lambda_0^{-1}) \times  \nonumber \\
  \prod_{i=1}^N \mathcal{N}(x_n | Ax_{n-1} + B u_{n}, diag(\tau_1^{-1}))\mbox{ ,} \label{eqn:Transition}
 \end{eqnarray}
   
    
    where $x_0$ is an auxiliary initial state with mean $m_0$ and a precision matrix of $\Lambda_0$ (the matrix inverse of the covariance matrix). The emission probability is given by  
  
    \begin{equation}
    P(Y | C, X , \tau) = \prod_{n=1}^N \mathcal{N}(y_n | C x_n, diag(\tau^{-1})) \mbox{ .}\label{eqn:Emission}
    \end{equation}
   
   
   
   
   Here $Y$ is a normal distribution with mean\textbf{ CX }and a covariance matrix with $diag(\tau^{-1})$. The covariance matrix \textbf{R} is a diagonal matrix as the noise is independent of the observed states $Y$. 
The graphical nature of the BSSM model is shown in Fig~\ref{fig:BSSM}, which is analogous to an Input-Output HMM~\cite{bengio1995input}.
    
  \begin{figure}[H]
  \includegraphics[scale=.25,width=.45\textwidth]{figs/BSSM.png}
  \caption{Bayesian State Space Model}
  \label{fig:BSSM} 
  \end{figure} 
  
  \subsection{{Problem Formulation}}  \label{subsec:Problem} We use an example to illustrate how to formulate a building's thermal equations and incorporate them into the proposed state space model framework. Figure~\ref{fig:TiTe} shows an equivalent circuit that describes the thermal dynamics of a house.

\begin{figure}[h]
\includegraphics[width=.45\textwidth]{figs/TiTe}
\caption{TiTe circuit model}
\label{fig:TiTe}
\end{figure}
  
  In this example, called the $TiTe$ model, we assume that there are two latent state spaces $Ti$ and $Te$ that describes the indoor and envelope temperatures. The thermal dynamics is represented by a set of stochastic differential equations derived from the equivalent assumption. The equations of the process are given by: 
  
   \begin{flalign}
   dT_i &= \frac{1}{R_{ie}C_i} (T_e - T_i) dt + \frac{1}{C_i}\Phi_hdt + \frac{A_w }{C_i}\Phi_s dt +  \sigma_i d\omega_i \\
   dT_e &= \frac{1}{R_{ie}C_e} (T_i - T_e) dt +  \frac{1}{R_{Bea}C_e} (T_a - T_e) dt   +  \sigma_e  d\omega_e \\
   Y_k &= T_{i_k} + e_k\mbox{ ,}
   \end{flalign}
 

 where \textit{t} is the time, \textit{$R_{ie}$} is the thermal resistance between the interior and the building envelope, \textit{$R_{ea}$} is the thermal resistance between the building envelope and the ambient air, $C_i$ is the heat capacity of the interior, $C_e$ is the heat capacity of the building envelope, $\Phi_h$ is the energy flux from the heating system, $A_w$ is the effective window area, $\Phi_s$ is the energy flux from solar radiation, $T_a$ is the ambient air temperature, $\{\omega_{i,t}\}$ and $\{\omega_{e,t}\}$ are standard Wiener processes with variances $\sigma_i$ and $\sigma_e$  respectively, where $t$ is the point in time of a measurement. $Y_t$ is the indoor temperature, $T_{i_k}$ is the measured interior and $e_k$ is the measurement error, which is assumed to be a Gaussian white noise process. Converting the differential equations (Eqns 5--7) as difference equations we get the transition and emission matrix form as:\\
 

  \begin{flalign}
   \begin{bmatrix} Ti(t+1) \\ Te(t+1)\end{bmatrix} &=
\begin{bmatrix}
    1 -  \frac{1}{R_{ie}C_i}    &  \frac{1}{R_{ie}C_i}   \\
   \frac{1}{R_{ie}C_e}     &    1 -  \frac{1}{R_{ie}C_e} -  \frac{1}{R_{ia}C_e}  
\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix}  \nonumber \\ 
&+ \begin{bmatrix}
    0   &  \frac{1}{C_i} &   \frac{A_{w}}{C_i} \\
   \frac{1}{R_{ia}C_e}     &    0 & 0
\end{bmatrix}\times \begin{bmatrix} Ta(t+1) \\ \Phi_h(t+1) \\ \Phi_s(t+1) \end{bmatrix}  + \begin{bmatrix}
   \sigma_{i}    &  0   \\
   0   &    \sigma_{e}  
\end{bmatrix} \label{eqn:trans}  \\
     Y(t)  &=  \begin{bmatrix} 1 & 0\end{bmatrix} \times \begin{bmatrix} Ti(t) \\ Te(t)\end{bmatrix} + \sigma \mbox{ .} \label{eqn:emis}
  \end{flalign}  
  \normalsize
  
  
   Eqn~\ref{eqn:trans} is the state transition of the dynamic system and is equivalent to the general form as presented in Eqn~\ref{eqn:stateEvolution} that gives us the transition probability, i.e $P(x_{t+1} | x_t)$ $\sim$ $\mathcal{N}(AX + BU, \Sigma_w)$ (Eqn~\ref{eqn:Transition}). Similarly,  Eqn~\ref{eqn:emis} is equivalent to the measurement equation provided by Eqn~\ref{eqn:obs} that gives us the emission probability (Eqn~\ref{eqn:Emission}).  In Eqn~\ref{eqn:trans}, the first two matrices models the physical dynamics and the third matrix is the measure of stochasticity in the data. Similarly, in Eqn~\ref{eqn:emis}, the first matrix is the measurement equation and $\sigma$ is the error in measurement. In the base case, we assume an uninformative Gamma prior over the model parameters  and the hyper-parameters of the gamma distribution are automatic relevance determination (ARD) parameters, which prune out components that are not significant enough. We provide broad priors to the gamma distribution by setting the shape and rate to a very small value~\cite{beal2003variational}. Thus parameters are given as   $\mathbf{R} \sim \Gamma(\alpha = \delta, \beta = \delta)$,
    $\mathbf{C} \sim \Gamma(\alpha = \delta, \beta = \delta)$, 
    $\mathbf{Aw} \sim \Gamma(\alpha = \delta, \beta = \delta)$,  where $\delta$ is a very small value. We also impose a bound on the parameters, which can help by limiting the parameters to certain reasonable ranges. We formulate other instantiations of the physical models in the case studies presented in Section 4.1.2. 
 \subsection{{Bayesian Inference}}
 \label{subsec:Inference}
 \indent   Bayesian inference recovers the posterior distribution over parameters and latent variables of the model, which can hence be used to perform prediction. While exact solutions can be achieved for some basic models, computing the posterior distribution is generally an intractable problem, in which case approximate inference is needed.\\
\indent \textbf{Markov chain Monte Carlo (MCMC)} algorithms are a widely applied method for approximate inference, which aims to estimate the posterior using a collection of samples drawn from an appropriate Markov chain.  Hamiltonian Monte Carlo (HMC)~\cite{neal2011mcmc} algorithms such as NUTS avoid the random walk behavior by taking a series of steps informed by first-order gradient information. These features allow it to converge to high-dimensional target distributions much more quickly than simpler methods such as random walk Metropolis Hastings~\cite{yildirim2012bayesian}.  The No U-Turn Sampler (NUTS)~\cite{hoffman2014no} uses a recursive algorithm to build a set of likely candidate points that span a range of the target distribution, stopping automatically when it starts to backtrack and retrace its steps, which prevents the revisiting of previously explored paths. In this work, we select the NUTS sampler for inference. \\  
\indent Another option is \textbf{Variational Inference}, which is a class of algorithms that are deterministic alternatives to MCMC. This reduces inference tasks to an optimization problem~\cite{blei2017variational}. In a probabilistic latent model setting, Y is the observed data, X is the latent variable space and $\theta$ the model parameters. An approximating distribution $q(X,\theta)$ over the latent variables and parameters, called the \emph{variational distribution}, is constructed to approximate the posterior. The objective is to reduce the ``gap'' between the variational and the posterior distribution. This gap is given by the Kullback-Leibler divergence, which is the relative entropy between the two distributions, given as:


    \begin{align} \label{eqn:KL}
      KL (q(X,\theta) || p(X, \theta | Y)) \nonumber = \mathbb{E}_q  \Big \lbrack log \: \frac{q(X,\theta)}{p(X, \theta | Y)} \Big \rbrack    \nonumber \\
       = \mathbb{E}_q \lbrack log\: q(X,\theta)\rbrack -  \mathbb{E}_q \lbrack log\: p(X, \theta, Y) \rbrack + log\: p(Y) \mbox{ .}  \\\nonumber
    \end{align}
   \normalsize
    
   In Eqn~\ref{eqn:KL}, $log\: p(Y)$ is independent of the distribution $q(X, \theta )$, so minimizing Eqn~\ref{eqn:KL} is equivalent to maximizing: 
   
\begin{align} \label{eqn:ELBO}
     \mathbf{L}(q)  = \mathbb{E}_q  \lbrack log\: p(X, \theta, Y) \rbrack -\mathbb{E}_q \lbrack log\: q(X,\theta)\rbrack  \nonumber \\
     = \mathbb{E}_q  \lbrack log\: p(X, \theta, Y) \rbrack + H(q) \mbox{ .} \\\nonumber
\end{align}
 \normalsize

\indent Using Jensen's inequality, $\mathbf{L}(q)$ can be shown to be a lower bound on $\log\: p(Y)$, and is hence known as the Evidence Lower Bound (ELBO). To make inference tractable, we make simplifying assumptions on $q$.  The most commonly used assumption is the mean-field approximation, which assumes that the latent variables are independent of each other. Thus the variational distribution with $N$ latent variables is assumed factorized as $q(X,\theta)   =  q(\theta)\prod_{i=1}^Nq(X_i) $. Traditionally, a Variational Inference algorithm requires developing and implementing model specific optimization routines. Automatic Differentiation Variational Inference (ADVI)~\cite{kucukelbir2017automatic} proposes an automatic solution to posterior inference. ADVI first transforms the model into one with unconstrained real-valued latent variables. It then recasts the gradient of the variational objective function as an expectation over \textbf{q}.  This involves the gradient of the log of the joint likelihood with respect to the latent variable $\bigtriangledown_{\theta}\;log\;p(x,\theta)$, which is computed using reverse-mode automatic differentiation~\cite{maclaurin2016modeling}. This gradient term is applied to optimize the parameters using a stochastic gradient descent approach.  \\
\indent It is important to note the underlying assumptions of ADVI. It factors the posterior distribution such that all the state variables are statistically independent, following the mean-field approximation. For a highly correlated posterior, e.g. in state space models, where the intuition is that  $x_{t+1} \sim N(x_{t}, \theta)$ will be highly correlated with $x_t$, the mean-field assumption is rather unrealistic. The method can still work well in practice, however, as the (uncorrelated) $q$ is fit to the (correlated) $p$, thereby exploiting dependencies, even though they are not ultimately encoded in $q$. NUTS, on the other hand, is very good at exploring a correlated, high-dimensional distribution, but can suffer in both run-time and convergence speed versus ADVI. We empirically evaluate the effectiveness of these approximations by comparing the parameters inferred by both the methods.
 

  \subsection{{Model Criticism }}
  
Model criticism requires tests for convergence   and testing goodness of fit on held out data. Since the primary objective of the study is to obtain the estimated parameter values, we also inspect the credible interval of the parameters. If the region is too wide we infer that the uncertainty in estimation is high.  \\ 
\indent \textbf{Convergence Diagnostics:} We select the \textit{Gelman-Rubin diagnostic}~\cite{gelman2011inference}, which checks for the lack of convergence by comparing the variance between multiple chains to the variance within each chain. Convergence is more straightforward to analyze for Variational Inference. The convergence criterion is simply to iterate until the ELBO no longer increases. \\ 
\indent \textbf{Goodness of fit} is tested using \emph{posterior predictive checks}, which are performed by simulating replicated data under the fitted model and then comparing these to the observed data to look for systematic discrepancies between real and simulated data~\cite{gelman2013bayesian}.\\ 
\indent \textbf{ Credible Interval:} The motivation behind using a Bayesian approach is to find the range of possible values for the building parameters. A standard measure of confidence in some (scalar) quantity $\theta$ is the ``width'' of its posterior distribution. This can be measured using a 100(1 - $\alpha$)\% \emph{credible interval}, where we select $\alpha$ as 0.05 to estimate parameters with a 95\% probability,
   \begin{equation}    
   C_{\alpha}(D)=(	l , u) : P(	 l \leq \theta \leq u| Y) = 1 -  \alpha \mbox{ ,}
   \end{equation}
    where the interval for a parameter is bounded by (l,u) with a probability $1-\alpha$. The credible interval is a Bayesian alternative to a frequentist confidence interval. A frequentist keeps the parameters fixed and varies the confidence interval whereas a Bayesian approach is to keep the credible region fixed and vary the model parameters. 
    
    
    
   \subsection{{Application of the Models}}
   
     
    \subsubsection{{Exploration}}

    In terms of building modeling, we are primarily interested in learning the different \textbf{R} and \textbf{C} parameters. As we consider different multi-state lumped models, the cardinality of the sets \textbf{R} and \textbf{C} may vary but the overall values should remain the same. To find the composite resistance of the equivalent circuit, the resistance and capacitance are obtained by Kirchoff's law. However, the simple addition or geometric sum required to compute the composite parameters cannot straightforwardly be done as Bayesian Inference provides random variables rather than scalar quantities. The distribution of the sum of two random variables can be obtained by the  convolution of their density functions.  
  

\begin{algorithm}
\caption{Indoor Temperature Forecast}
\label{alg:Forecast}
\begin{algorithmic}[1]
\Procedure{Forecast\text{ }} {\emph{Input}: Distribution of the model parameters $\theta=\{\mathbf{R} , \mathbf{C}, \mathbf{A}, \mathbf{X}_{T}\}$, time window of forecast $K$}
\State Set start temperature state to $X_T$ 
\State  \{$R_i$ , $C_i$, $A_i$\} <- Draw N Sample(R, C, A) 
\For{i in 1 : N}
\State   $X^{(i)}_{T+1:T+K}$ $\leftarrow$ $BSSM(X_T, R_i , C_i, A_i)$
\EndFor
\State Mean Prediction $\leftarrow$ $\mathbf{E}\{ X^{(i)}_{T+1:T+K} \}$
\State Credible Interval $\leftarrow$ \{$Max(X^{(i)}_{T+1:T+K})$ , $Min(X^{(i)}_{T+1:T+K})$\}
\EndProcedure
\end{algorithmic}
\end{algorithm}



\subsubsection{Forecasting}
      
  We perform 24 hour ahead forecast, after learning the parameters of the model. We assume that a outdoor temperature forecast data is given to us and we assumed that the HVAC is operational in the last known mode. The forecasting and prediction of HVAC time is given in Algorithm~\ref{alg:Forecast}.    When the HVAC is set to a particular temperature and assuming that it is not changed within the horizon of the forecast, then the indoor temperature will be centered around the set-point in a range known as the thermostat hysteresis setting. In general, the range is $\pm$ $\delta$ lies within 0.5 -- 1 $^\circ$F. We sample from the estimated parameters' distributions to obtain the forecasting interval.
  
  
\subsection{Implementation}
   
   We implemented the Bayesian State Space model using the PyMC3 probabilistic programming library in Python~\cite{PYMC3}. PyMC3 is built on  Theano~\cite{Theano} and has built-in implementations for MCMC algorithms and Variational Inference methods. We formulated the different components of the state space model and set the prior distributions for the model parameters. We deployed our methods on a system with 16 GB RAM system and I7 processor. The initial version of the codes is available in the \href{https://github.com/Nilavro/BSSPy}{\color{blue} BSSP} Github repository.  
   



==> EEnergy Arxiv/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> EEnergy Arxiv/Related.tex <==


\section{{Related Works}}   
\label{sec:Related}
  In this section, we review the previous works in three major related areas -- parametric modeling of buildings' thermal dynamics, techniques for parameter estimation, and a brief review of techniques for Bayesian inference.  \\
\indent \textbf{Parametric modeling of buildings' thermal dynamics}  helps to understand a  building's quality with few parameters. There are three approaches for modeling buildings' thermal dynamics -- \emph{White-box}, \emph{Black-box } and \emph{Gray-box} modeling. \emph{White-box} approach models all physical processes of a building~\cite{HONG2000347,KIRCHER2015454} by formulating exact system dynamics. Such deterministic models are difficult to construct as the exact dynamics are often unavailable and due to the presence of noise in the data, arising from unaccounted factors. \emph{Black-box modeling} approaches, such as regression, neural networks etc., are applied to model indoor temperature as a function of observed data, much like outdoor temperature~\cite{nielsen2010analysis}. However they do not describe the generative process and thus isn't effective for interpretation. A \emph{gray-box model} is  a combination of prior physical knowledge and statistical approaches. The heat dynamics of the building was formulated  using several equivalent models of varying complexity in~\cite{bacher2011identifying}, that  estimated the insulation and the thermal mass of a building. An extension of such an approach included the effect of wind speed on infiltration is proposed in~\cite{EstimationBuildsys}, and expansionary effect of air with temperature changes was modeled in~\cite{siemann2013performance}.    \\ 
\indent  \textbf{ Parameter estimation} for the gray-box model was performed in~\cite{KRISTENSEN2004225} by  maximum likelihood estimation (MLE) and maximum a posteriori estimation (MAP). An extension of the approach~\cite{ghosh2015modeling}, chose a simpler model to represent the dynamics and learned the residuals separately with Gaussian priors. Other works have focused on optimization based techniques~\cite{Optimization,EstimationBuildsys}, where the objective is to minimize  deviation between measurements and predictions from the model. Although, these approaches are simpler, they do not incorporate noise estimation in the equations. Alternatively, a Bayesian approach offers a natural way of dealing with parameter uncertainty in a state space model~\cite{gordon1993novel, geweke2001bayesian}. Bayesian methods have been widely used for the closely related problem of building energy modeling ~\cite{LI2016194,heo2012calibration,kim2013stochastic,kristensen2017bayesian}, but have been less well studied in the context of \emph{thermal modeling for buildings}~\cite{bacher2011identifying,rouchier2018calibration}.  A majority of previous  works have applied the Metropolis-Hastings algorithm for Bayesian inference ~\cite{rouchier2018calibration,heo2012calibration,kim2013stochastic,LI2016194,kristensen2017bayesian} which is ill-fitted for the specific problem as it takes a large number of steps to achieve convergence. The No U-Turn sampler (NUTS) showed better results~\cite{chong2017bayesian} for parameter estimation in a related problem, building energy models, so we choose the latter.\\
\indent  \textbf{Bayesian Inference}, as performed in the previous works, used uninformed uniform priors and/or Normal priors for the model parameters~\cite{bacher2011identifying,rouchier2018calibration}. Such assumptions do not hold true as the parameters typically have non-Normal distributions. Non-normal priors do not have conjugacy with the  likelihood, and analytical solutions of the posterior distribution are not possible. In such cases, algorithms that do not rely on conjugacy become important such as MCMC and Variational Inference. MCMC algorithms are capable of overcoming this problem but are time-consuming. Alternatively, Variational Inference~\cite{beal2003variational, luttinen2013fast} is an approximate inference that derives a lower bound for the marginal likelihood which can be optimized using stochastic gradient descent. In our experiments, we use the Mean Field Variational Inference and find that it provides similar parameter estimation to MCMC algorithms. 

 


==> EEnergy Arxiv/Rest.tex <==
\section*{Appendix}
\appendix
%Appendix A
\section{Detailed Results}

In this section, we list the detailed result which couldn't be included in the main paper.
 
\subsection{Use Case I}
\label{Ap:UC1}

 \subsubsection{Data Plot and Discussion}
    Figure~\ref{fig:CTSM} describes the data provided in CTSM~\cite{juhl2017grey}. The data is collected for six days and indoor 
    
    \begin{figure*}[!htp]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/Fig1_data}
    \caption{CTSM Dataset}
    \label{fig:CTSM}
    \end{figure*}   
    
 
\begin{figure*}[ht!]
\centering     
\begin{subfigure}{.4\textwidth}
\includegraphics[width=\textwidth]{figs/KalmanPeriodgram}
\caption{Kalman Periodgram}
\label{fig:BadModel1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\includegraphics[ width=\textwidth]{figs/ACFKalman}
\caption{Kalman Periodgram}
\label{fig:BadModel2}
\end{subfigure}    
\caption{Analysis of Kalman Filter Residuals}
\begin{subfigure}{.4\textwidth}
\includegraphics[width=\textwidth]{figs/PeriodgramBayes}
\caption{Bayesian Periodgram}
\label{fig:BayesPeriod}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\includegraphics[ width=\textwidth]{figs/ACFBayes}
\caption{Bayesian ACF}
\label{fig:BayesACF}
\end{subfigure}    

\caption{Analysis of Bayesian Residuals Residuals}
\end{figure*} 


\begin{figure*}[ht!]
\centering     
\begin{subfigure}{.49\textwidth}
\includegraphics[ width=\textwidth]{figs/indoor}
\caption{Indoor Temperature Sensor Data}
\label{fig:Indoor}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\includegraphics[ width=\textwidth]{figs/outdoor}
\caption{Outdoor Temperature: Original and filtered}
\label{fig:Temps}
\end{subfigure}    
\begin{subfigure}{.25\textwidth}
\includegraphics[ width=\textwidth]{figs/sensors}
\caption{Temperature Sensor Correlation}
\label{fig:Corr}
\end{subfigure}  
\hfill
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/indoor_anomaly}
\caption{Indoor Temperature Sensor Data Aberration} 
\label{fig:indooranomaly}
\end{subfigure}   
\hfill
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/HVAC}
\caption{HVAC Cycling}
\label{fig:HVAC}
\end{subfigure}  
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/ELBO}
\caption{Convergence Plots}
\label{fig:ELBO}
\end{subfigure} 
\caption{Collected Data}
\end{figure*} 


\begin{table*}[!ht]
\scriptsize
\caption{Results of the Bayesian Estimation}
\label{Table:BayesianParameters}
\begin{tabular}{||p{0.5cm}|p{0.4cm}|p{0.5cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm} |p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.7cm}|p{0.7cm}|p{1cm}|p{1cm}||} 
\hline
Models &     RMSE & Aw & Ae & Ria & Rie & Rih   & Rim & Rea & Ci & Ce & Cm & Ch  & Total R & Total C\\ [0.5ex] 
\hline\hline 
Ti & 0.2   & 10.62, 41.30 & & 5.15, 0.70 &   &      &   &   & 25.75, 4.95 &   &   &    &    &    \\
\hline
TiTh & 0.036 & 4.94, 17.13 & & 31.49, 10.45
 &  & 21.16, 9.87  &   &   &   & 44.47, 16.89 &      &  94.85, 6.00  &     &   \\
\hline
TiTe &  0.119 & 8.64, 15.44 & &   & 2.09, 0.006
  &   &      & 2.03, 0.006  & 29.65, 4.16
 &  0.99, 0.02 &   &    &     &   \\
\hline
TiTm & 0.03  &  3.92, 12.03 &   & 10.12, 0.61  &      &   &  7.25, 0.15 &   & 24.68, 0.50
 &   & 94.24, 6.90  &    &     &   \\
\hline
TiTeTh & 0.068 & 10.19, 27.60 & &  & 2.08, 0.004
 & 32.56, 17.66  &      & 2.09, 0.004
  & 97.00, 4.33  & 0.96, 0.01  &   &   23.75, 16.19 &     &   \\
\hline
TiTeThAe & 0.015  & 5.649, 20.76 & 5.289, 20.54 & 0.29, 0.0009 &  4.12,  0.0045 & 0.2898, 0.0009  &      &    1.177, 0.0013  & 23.547, 0.984 &  1.093, 0.009 &   & 3.582, 0.038  &     &   \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\caption{Results of the Kalman Filter Estimation}
\label{Table:KalmanParameters}
\begin{tabular}{||p{2cm}|p{1cm}|p{1cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.6cm}|p{0.6cm}|p{0.5cm}|p{0.5cm}||} 
\hline
Models & RMSE & Lik & Aw & Ria & Rie & Rih & Ris & Rim & Rea & Ci & Ce & Cm & Ch  & Total R & Total C\\ [0.5ex] 
\hline\hline 
Ti & 5.39 & 2463.47 &  7.9  & 5.29   &   &   &   &   &   & 2.06 &   &   &    & 5.29   &  2.06 \\
\hline
TiTe & 1.52 & 3643.08 &  23.78  &     &  2.70 &   &   &   &  0.93 & 5.71 & 1.65   &   &    &   &   \\
\hline
TiTh & 0.98 & 3910.32 &  6.22  &  5.31   &   & 0.64  &   &   &   & 1.36 & 1.65   &   &  0.31  &   &   \\
\hline
TiTm & 1.52 & 3641.32 &  6.22  &  5.31   &   & 0.64  &   &   &   & 1.36 & 1.65   &   &  0.31  &   &   \\
\hline
TiTeTh & 0.16 & 5516.38  &  5.63  &      & 0.86 & 119.03  &   &   &  4.53 & 1.07 & 2.92  &   &  0.001  &   &   \\
\hline
TiTmTeThTs & 0.21 &  5268.35  &    &      &   &    &   &   &   &   &    &   &    &   &   \\
\hline
\end{tabular}
\end{table*}



\textbf{Updates:}
\begin{itemize}

\item \textbf{Home data cleaning and observations:}
\begin{itemize}

\item \textbf{Temperature:} Spiky noise data. 
Hourly data. EWMA. Cubic interpolation.

\item \textbf{HVAC:} Push ON mechanism. Fill the values. Bring it to 10 min. Val > .4 == 1

\item \textbf{Temp Sensors:} Staircase data. Sample down 10 min. EWMA. \\
Mean signal. Correlation with individual signals. Do a weighted average - single sensor equivalent. 
Room wise model - individual sensor. \textbf{Fails} - C is dependent on Volume. Heat distribution is same. Local influencing factors not considered. 


\item \textbf{Observation:} HVAC sensor temp not same as the temp sensor in proximity.

\item Experiments: Comparing MCMC(exact) and ADVI(approximate). MCMC has diagnostic test.
ADVI is gradient optimization so we get a plot of convergence. We compare estimated parameters. Perform forecasting. [Model checks]. Comparing Hierarchical model tests.

Take two different segments of data and learn parameters to figure out how much do they deviate.





\end{itemize}

\end{itemize}


\begin{tabular}{cc|c|c|c|c|l}
\cline{3-6}
& & \multicolumn{4}{ c| }{Primes} \\ \cline{3-6}
& & 2 & 3 & 5 & 7 \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{Powers} } &
\multicolumn{1}{ |c| }{504} & 3 & 2 & 0 & 1 &     \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{540} & 2 & 3 & 1 & 0 &     \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{Powers} } &
\multicolumn{1}{ |c| }{gcd} & 2 & 2 & 0 & 0 & min \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{lcm} & 3 & 3 & 1 & 1 & max \\ \cline{1-6}
\end{tabular}

\begin{table}[!htb]
    \caption{Global caption}
    \begin{minipage}{1.5\linewidth}
      \caption{}
      \centering
    \begin{tabular}{|p{0.8cm} |c|c|c|c|c|c|c|c|c|c|c|p{0.8cm}|c|}
\hline
Model             & Method &   R &   C & Ria & Rie & Rea & Rih & Ci & Ce & Ch & Aw & NRMSE & $R^2$ \\ \hline
Ti                & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
TiTe              & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
TiTeTh            & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\end{tabular}
    \end{minipage}%
    \begin{minipage}{1\linewidth}
      \centering
        \caption{}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Model                 & Method &  R &  C & Ria & Rie & Rea & Ci & Ce & $\alpha$ \\ \hline
\multirow{2}{*}{Ti}   & KF     &         &         &     &     &     &    &    &          \\ \cline{2-10} 
                      & BSSM   &         &         &     &     &     &    &    &          \\ \hline
\multirow{2}{*}{TiTe} & KF     &         &         &     &     &     &    &    &          \\ \cline{2-10} 
                      & BSSM   &         &         &     &     &     &    &    &          \\ \hline
\end{tabular}
    \end{minipage} 
\end{table}


\begin{table}[]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\cline{1-8} \cline{10-10}
Model                 & Method & Total R & Total C & Ria & Rie & Rea & Ci &  & $\alpha$ \\ \cline{1-8} \cline{10-10} 
\multirow{2}{*}{Ti}   & KF     &         &         &     &     &     &    &  &          \\ \cline{2-8} \cline{10-10} 
                      & ADVI   &         &         &     &     &     &    &  &          \\ \cline{1-8} \cline{10-10} 
\multirow{2}{*}{TiTe} & KF     &         &         &     &     &     &    &  &          \\ \cline{2-8} \cline{10-10} 
                      & ADVI   &         &         &     &     &     &    &  &          \\ \cline{1-8} \cline{10-10} 
\end{tabular}
\end{table}


\subsubsection{Dataset}
\label{data:col}

    We collected temperature data from a townhouse, inhabited by three residents and the data was collected in an uncontrolled environment. The townhouse has two floors and a basement. The dataset consist of : Weather, HVAC and Indoor Temperature. \emph{Weather:} The simplest data to collect on our experimental location was weather data. We used the free weather data API at \href{DarkSky.net}{\color{blue} DarkSky}  to collect data for various weather related data (primarily the outdoor temperature) based on the coordinates of our experimental residence. This data has a 1-hour resolution. \emph{HVAC:} Our experimental location was also furnished with a \href{ https://nest.com/thermostats/}{\color{blue} Nest thermostat}. This gave us an API to collect the HVAC mode (heating or cooling), the on/off state of the circulating fan, the target indoor temperature, the indoor humidity, the on/off state of the heating or cooling system, and the indoor temperature at the thermostat. These data were updated in a ``push'' fashion within seconds as they changed. \emph{Sensor network:} Our third source of data at our experimental location was a small network of consumer, off the shelf, wireless sensor devices. We deployed \href{https://products.z-wavealliance.org/products/1170}{\color{blue} Z-wave Gen5 MultiSensors} into each of five rooms in the home to collect additional indoor temperature measurements. The sensors report with a precision of $0.1\degree F$ each time the temperature changes. These sensors communicate wirelessly through a \href{http://www.z-wave.com/}{\color{blue} Z-Wave} 
mesh network to a base station. The base station was a  \href{https://www.raspberrypi.org/products/raspberry-pi-3-model-b/}{\color{blue} RaspberryPi 3} with a \href{https://aeotec.com/z-wave-usb-stick}{\color{blue} Z-Stick} USB dongle. The base station ran \href{https://docs.openhab.org/}{\color{blue} OpenHAB2},a free software home automation control software, to communicate with the Z-Wave network, collect the sensor data, and cache the data locally. Our software on the base station uploaded the data to our server via a RESTful API. The data were secured in transit with TLS 1.2.  The data is collected from December 6, 2017 and we are actively collecting it now. 























==> EEnergy Arxiv/natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

==> Rest.tex <==
\section*{Appendix}
\appendix
%Appendix A
\section{Detailed Results}

In this section, we list the detailed result which couldn't be included in the main paper.
 
\subsection{Use Case I}
\label{Ap:UC1}

 \subsubsection{Data Plot and Discussion}
    Figure~\ref{fig:CTSM} describes the data provided in CTSM~\cite{juhl2017grey}. The data is collected for six days and indoor 
    
    \begin{figure*}[!htp]
    \centering
    \includegraphics[width=0.8\textwidth]{figs/Fig1_data}
    \caption{CTSM Dataset}
    \label{fig:CTSM}
    \end{figure*}   
    
 
\begin{figure*}[ht!]
\centering     
\begin{subfigure}{.4\textwidth}
\includegraphics[width=\textwidth]{figs/KalmanPeriodgram}
\caption{Kalman Periodgram}
\label{fig:BadModel1}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\includegraphics[ width=\textwidth]{figs/ACFKalman}
\caption{Kalman Periodgram}
\label{fig:BadModel2}
\end{subfigure}    
\caption{Analysis of Kalman Filter Residuals}
\begin{subfigure}{.4\textwidth}
\includegraphics[width=\textwidth]{figs/PeriodgramBayes}
\caption{Bayesian Periodgram}
\label{fig:BayesPeriod}
\end{subfigure}
\begin{subfigure}{.4\textwidth}
\includegraphics[ width=\textwidth]{figs/ACFBayes}
\caption{Bayesian ACF}
\label{fig:BayesACF}
\end{subfigure}    

\caption{Analysis of Bayesian Residuals Residuals}
\end{figure*} 


\begin{figure*}[ht!]
\centering     
\begin{subfigure}{.49\textwidth}
\includegraphics[ width=\textwidth]{figs/indoor}
\caption{Indoor Temperature Sensor Data}
\label{fig:Indoor}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
\includegraphics[ width=\textwidth]{figs/outdoor}
\caption{Outdoor Temperature: Original and filtered}
\label{fig:Temps}
\end{subfigure}    
\begin{subfigure}{.25\textwidth}
\includegraphics[ width=\textwidth]{figs/sensors}
\caption{Temperature Sensor Correlation}
\label{fig:Corr}
\end{subfigure}  
\hfill
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/indoor_anomaly}
\caption{Indoor Temperature Sensor Data Aberration} 
\label{fig:indooranomaly}
\end{subfigure}   
\hfill
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/HVAC}
\caption{HVAC Cycling}
\label{fig:HVAC}
\end{subfigure}  
\begin{subfigure}{.35\textwidth}
\includegraphics[ width=\textwidth]{figs/ELBO}
\caption{Convergence Plots}
\label{fig:ELBO}
\end{subfigure} 
\caption{Collected Data}
\end{figure*} 


\begin{table*}[!ht]
\scriptsize
\caption{Results of the Bayesian Estimation}
\label{Table:BayesianParameters}
\begin{tabular}{||p{0.5cm}|p{0.4cm}|p{0.5cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm} |p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.7cm}|p{0.7cm}|p{1cm}|p{1cm}||} 
\hline
Models &     RMSE & Aw & Ae & Ria & Rie & Rih   & Rim & Rea & Ci & Ce & Cm & Ch  & Total R & Total C\\ [0.5ex] 
\hline\hline 
Ti & 0.2   & 10.62, 41.30 & & 5.15, 0.70 &   &      &   &   & 25.75, 4.95 &   &   &    &    &    \\
\hline
TiTh & 0.036 & 4.94, 17.13 & & 31.49, 10.45
 &  & 21.16, 9.87  &   &   &   & 44.47, 16.89 &      &  94.85, 6.00  &     &   \\
\hline
TiTe &  0.119 & 8.64, 15.44 & &   & 2.09, 0.006
  &   &      & 2.03, 0.006  & 29.65, 4.16
 &  0.99, 0.02 &   &    &     &   \\
\hline
TiTm & 0.03  &  3.92, 12.03 &   & 10.12, 0.61  &      &   &  7.25, 0.15 &   & 24.68, 0.50
 &   & 94.24, 6.90  &    &     &   \\
\hline
TiTeTh & 0.068 & 10.19, 27.60 & &  & 2.08, 0.004
 & 32.56, 17.66  &      & 2.09, 0.004
  & 97.00, 4.33  & 0.96, 0.01  &   &   23.75, 16.19 &     &   \\
\hline
TiTeThAe & 0.015  & 5.649, 20.76 & 5.289, 20.54 & 0.29, 0.0009 &  4.12,  0.0045 & 0.2898, 0.0009  &      &    1.177, 0.0013  & 23.547, 0.984 &  1.093, 0.009 &   & 3.582, 0.038  &     &   \\
\hline
\end{tabular}
\end{table*}

\begin{table*}[!ht]
\caption{Results of the Kalman Filter Estimation}
\label{Table:KalmanParameters}
\begin{tabular}{||p{2cm}|p{1cm}|p{1cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.7cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.8cm}|p{0.6cm}|p{0.6cm}|p{0.5cm}|p{0.5cm}||} 
\hline
Models & RMSE & Lik & Aw & Ria & Rie & Rih & Ris & Rim & Rea & Ci & Ce & Cm & Ch  & Total R & Total C\\ [0.5ex] 
\hline\hline 
Ti & 5.39 & 2463.47 &  7.9  & 5.29   &   &   &   &   &   & 2.06 &   &   &    & 5.29   &  2.06 \\
\hline
TiTe & 1.52 & 3643.08 &  23.78  &     &  2.70 &   &   &   &  0.93 & 5.71 & 1.65   &   &    &   &   \\
\hline
TiTh & 0.98 & 3910.32 &  6.22  &  5.31   &   & 0.64  &   &   &   & 1.36 & 1.65   &   &  0.31  &   &   \\
\hline
TiTm & 1.52 & 3641.32 &  6.22  &  5.31   &   & 0.64  &   &   &   & 1.36 & 1.65   &   &  0.31  &   &   \\
\hline
TiTeTh & 0.16 & 5516.38  &  5.63  &      & 0.86 & 119.03  &   &   &  4.53 & 1.07 & 2.92  &   &  0.001  &   &   \\
\hline
TiTmTeThTs & 0.21 &  5268.35  &    &      &   &    &   &   &   &   &    &   &    &   &   \\
\hline
\end{tabular}
\end{table*}



\textbf{Updates:}
\begin{itemize}

\item \textbf{Home data cleaning and observations:}
\begin{itemize}

\item \textbf{Temperature:} Spiky noise data. 
Hourly data. EWMA. Cubic interpolation.

\item \textbf{HVAC:} Push ON mechanism. Fill the values. Bring it to 10 min. Val > .4 == 1

\item \textbf{Temp Sensors:} Staircase data. Sample down 10 min. EWMA. \\
Mean signal. Correlation with individual signals. Do a weighted average - single sensor equivalent. 
Room wise model - individual sensor. \textbf{Fails} - C is dependent on Volume. Heat distribution is same. Local influencing factors not considered. 


\item \textbf{Observation:} HVAC sensor temp not same as the temp sensor in proximity.

\item Experiments: Comparing MCMC(exact) and ADVI(approximate). MCMC has diagnostic test.
ADVI is gradient optimization so we get a plot of convergence. We compare estimated parameters. Perform forecasting. [Model checks]. Comparing Hierarchical model tests.

Take two different segments of data and learn parameters to figure out how much do they deviate.





\end{itemize}

\end{itemize}


\begin{tabular}{cc|c|c|c|c|l}
\cline{3-6}
& & \multicolumn{4}{ c| }{Primes} \\ \cline{3-6}
& & 2 & 3 & 5 & 7 \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{Powers} } &
\multicolumn{1}{ |c| }{504} & 3 & 2 & 0 & 1 &     \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{540} & 2 & 3 & 1 & 0 &     \\ \cline{1-6}
\multicolumn{1}{ |c  }{\multirow{2}{*}{Powers} } &
\multicolumn{1}{ |c| }{gcd} & 2 & 2 & 0 & 0 & min \\ \cline{2-6}
\multicolumn{1}{ |c  }{}                        &
\multicolumn{1}{ |c| }{lcm} & 3 & 3 & 1 & 1 & max \\ \cline{1-6}
\end{tabular}

\begin{table}[!htb]
    \caption{Global caption}
    \begin{minipage}{1.5\linewidth}
      \caption{}
      \centering
    \begin{tabular}{|p{0.8cm} |c|c|c|c|c|c|c|c|c|c|c|p{0.8cm}|c|}
\hline
Model             & Method &   R &   C & Ria & Rie & Rea & Rih & Ci & Ce & Ch & Aw & NRMSE & $R^2$ \\ \hline
Ti                & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
TiTe              & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
TiTeTh            & KF     &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\multirow{2}{*}{} & MCMC   &         &         &     &     &     &     &    &    &    &    &       &       \\ \cline{2-14} 
                  & ADVI   &         &         &     &     &     &     &    &    &    &    &       &       \\ \hline
\end{tabular}
    \end{minipage}%
    \begin{minipage}{1\linewidth}
      \centering
        \caption{}
    \begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\hline
Model                 & Method &  R &  C & Ria & Rie & Rea & Ci & Ce & $\alpha$ \\ \hline
\multirow{2}{*}{Ti}   & KF     &         &         &     &     &     &    &    &          \\ \cline{2-10} 
                      & BSSM   &         &         &     &     &     &    &    &          \\ \hline
\multirow{2}{*}{TiTe} & KF     &         &         &     &     &     &    &    &          \\ \cline{2-10} 
                      & BSSM   &         &         &     &     &     &    &    &          \\ \hline
\end{tabular}
    \end{minipage} 
\end{table}


\begin{table}[]
\centering
\caption{My caption}
\label{my-label}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|}
\cline{1-8} \cline{10-10}
Model                 & Method & Total R & Total C & Ria & Rie & Rea & Ci &  & $\alpha$ \\ \cline{1-8} \cline{10-10} 
\multirow{2}{*}{Ti}   & KF     &         &         &     &     &     &    &  &          \\ \cline{2-8} \cline{10-10} 
                      & ADVI   &         &         &     &     &     &    &  &          \\ \cline{1-8} \cline{10-10} 
\multirow{2}{*}{TiTe} & KF     &         &         &     &     &     &    &  &          \\ \cline{2-8} \cline{10-10} 
                      & ADVI   &         &         &     &     &     &    &  &          \\ \cline{1-8} \cline{10-10} 
\end{tabular}
\end{table}


\subsubsection{Dataset}
\label{data:col}

    We collected temperature data from a townhouse, inhabited by three residents and the data was collected in an uncontrolled environment. The townhouse has two floors and a basement. The dataset consist of : Weather, HVAC and Indoor Temperature. \emph{Weather:} The simplest data to collect on our experimental location was weather data. We used the free weather data API at \href{DarkSky.net}{\color{blue} DarkSky}  to collect data for various weather related data (primarily the outdoor temperature) based on the coordinates of our experimental residence. This data has a 1-hour resolution. \emph{HVAC:} Our experimental location was also furnished with a \href{ https://nest.com/thermostats/}{\color{blue} Nest thermostat}. This gave us an API to collect the HVAC mode (heating or cooling), the on/off state of the circulating fan, the target indoor temperature, the indoor humidity, the on/off state of the heating or cooling system, and the indoor temperature at the thermostat. These data were updated in a ``push'' fashion within seconds as they changed. \emph{Sensor network:} Our third source of data at our experimental location was a small network of consumer, off the shelf, wireless sensor devices. We deployed \href{https://products.z-wavealliance.org/products/1170}{\color{blue} Z-wave Gen5 MultiSensors} into each of five rooms in the home to collect additional indoor temperature measurements. The sensors report with a precision of $0.1\degree F$ each time the temperature changes. These sensors communicate wirelessly through a \href{http://www.z-wave.com/}{\color{blue} Z-Wave} 
mesh network to a base station. The base station was a  \href{https://www.raspberrypi.org/products/raspberry-pi-3-model-b/}{\color{blue} RaspberryPi 3} with a \href{https://aeotec.com/z-wave-usb-stick}{\color{blue} Z-Stick} USB dongle. The base station ran \href{https://docs.openhab.org/}{\color{blue} OpenHAB2},a free software home automation control software, to communicate with the Z-Wave network, collect the sensor data, and cache the data locally. Our software on the base station uploaded the data to our server via a RESTful API. The data were secured in transit with TLS 1.2.  The data is collected from December 6, 2017 and we are actively collecting it now. 























==> natbib/README <==
                                 What is NATBIB?
                                 
It is a LaTeX (2e, with some support for 2.09) package to act as generalized
interface for standard and non-standard bibliographic style files (BibTeX).

It is intended primarily to produce author-year style citations from a variety
of non-standard .bst outputs; it therefore replaces the special and individual
packages that go along with such .bst files:
   apalike.sty    for    apalike.bst et al.
   newapa.sty            newapa.bst, 
   chicago.sty           chicago.bst, named.bst et al.
   harvard.sty           agsm.bst, dcu.bst, kluwer.bst et al.
   astron.sty            astron.bst, apa.bst, humanbio.bst, et al.
   authordate<n>.sty     authordate<n>.bst, aaai-named.bst
   
The above .bst files may also be used with natbib to produce author-year or 
numerical citations, so that switching from author-year to numerical is only 
a matter of selecting an option. 

The standard .bst files (plain et al) and other numerical citation .bst files
are also understood, but they can produce only numerical citations.
Replacement .bst files
   plainnat.bst
   abbrvnat.bst
   unsrtnat.bst
are provided to produce the same formatting of the reference list as the
standard equivalent, but allowing both author-year and numerical citations.

See my parallel custom-bib system for generating customized bst files.

For installation instructions and more details, see README.vxx.

Patrick W. Daly
Max-Planck-Institut f\"ur Sonnensystemforschung
D-37191 Katlenburg-Lindau, Germany
E-mail: daly@mps.mpg.de

